Long-Horizon Planning with Latent World Models via Graph Anchors

Latent world models plan in a compact latent space by predicting the outcomes of actions. Their planners judge a plan by the latent distance between its predicted end state and the goal image. We show that this distance fails in two distinct ways. First, it loses directional signal a few steps from the goal, causing distant goals to fail. Second, it weighs the robot arm over the manipulated object, causing manipulation to fail at contact. We measure both failures directly on recorded data by asking whether a lower latent distance corresponds to true progress toward the goal. Across five environments, six visual representations (including raw pixels and V-JEPA 2), and nine Meta-World tasks, this ranking test cleanly separates the two failures, and the graph distance to a goal predicts where closed-loop planning breaks down. Both failures share a single remedy: replacing the distant goal with a nearby target that lies on a recorded trajectory. We realize this principle with Graph Anchors, a training-free planner for frozen latent world models. It builds a sparse graph once over the model's own training frames and aims each planning step at a node a few moves ahead along the shortest path to the goal, keeping paths on recorded transitions wherever contact matters. On goals up to 400 steps away, Graph Anchors raise LeWM's success from 13% to 85% on PointMaze-Medium, from 8% to 87% on PointMaze-Large, and from 5% to 71% on Push-T, where stronger search toward the goal fails and where prior training-free planners break down under missing step horizons, subsampling shortcuts, or fragmented contact.

==> tables/abl_rows.tex <==
Full graph (k=10, $\tau$ = median, all data) & 86 & 86 \\
Temporal edges only (no neighbour edges) & 6 & 10/2 \\
$k=5$ neighbours & 80 & 80 \\
$k=20$ neighbours & 80 & 80 \\
Threshold $\tau$ at the 25th percentile & 74 & 74 \\
Threshold $\tau$ at the 75th percentile & 86 & 86 \\
50\% of the episodes & 84 & 86/82 \\
25\% of the episodes & 83 & 76/90 \\
10\% of the episodes & 79 & 80/78 \\
\midrule
LeWM planner, PointMaze-M, $d{=}200$: 300 $\to$ 900 CEM samples & 12 $\to$ 12 & \\
LeWM + min-over-plan, PointMaze-M, $d{=}200$: 300 $\to$ 900 CEM samples & 10 $\to$ 10 & \\
LeWM planner, Two-Room, $d{=}75$: 300 $\to$ 900 CEM samples & 28 $\to$ 36 & \\
LeWM + min-over-plan, Two-Room, $d{=}75$: 300 $\to$ 900 CEM samples & 54 $\to$ 56 & \\


==> tables/apdist_rows.tex <==
PointMaze-M, $d{=}100$ & 47 & 59 & 95 & 92 & 74 & 50 & 15 & 89 \\
PointMaze-M, $d{=}200$ & 29 & 31 & 54 & 81 & 70 & 48 & 11 & 87 \\
Two-Room, $d{=}75$ & 36 & 83 & -- & 96 & -- & 96 & 2 & 94 \\
PointMaze-L, $d{=}200$ & -- & 17 & -- & 16 & -- & 17 & -- & 73 \\
PointMaze-L, $d{=}400$ & -- & 11 & -- & 12 & -- & 14 & -- & 87 \\


==> tables/apoff_rows.tex <==
PointMaze-M, $d{=}100$ & 56 & 88 & 62 & 84 \\
PointMaze-M, $d{=}200$ & 34 & 80 & 54 & 92 \\
Two-Room, $d{=}50$ & 86 & 94 & 100 & 92 \\
Two-Room, $d{=}75$ & 82 & 98 & 94 & 94 \\


==> tables/budget_rows.tex <==
GCBC, 1 epoch (3 trainings) & 93 & 83 & 54 & 51 & 51 \\
GCBC, 4 epochs & 98 & 88 & 68 & 58 & 59 \\
GCIVL, 1 epoch & 30 & 4 & 2 & 0 & 16 \\
GCIVL, 4 epochs & 30 & 2 & 0 & 0 & 12 \\
PLDM, 5 epochs: planner & 28 & 8 & -- & 1 & 20 \\
\quad + min-over-plan & -- & 10 & -- & 1 & -- \\
\rowcolor{pactrow}\quad + graph anchors (ours) & -- & 33 & -- & 7 & 29 \\


==> tables/cmp_pml_head.tex <==
PointMaze-L & $d{=}50$ & $d{=}100$ & $d{=}200$ & $d{=}400$ & stitched \\


==> tables/cmp_pml_rows.tex <==
LeWM~\cite{maes2026leworldmodel} & 14\,{\scriptsize$\pm$3} & 15\,{\scriptsize$\pm$7} & 13\,{\scriptsize$\pm$4} & 8\,{\scriptsize$\pm$0} & 5\,{\scriptsize$\pm$1} \\
LeWM + min-over-plan & 44\,{\scriptsize$\pm$8} & 28\,{\scriptsize$\pm$3} & 23\,{\scriptsize$\pm$4} & 26\,{\scriptsize$\pm$6} & 17\,{\scriptsize$\pm$1} \\
\midrule
GCIVL~\cite{park2025ogbench} & 9\,{\scriptsize$\pm$1} & 8\,{\scriptsize$\pm$3} & 9\,{\scriptsize$\pm$1} & 1\,{\scriptsize$\pm$1} & 3\,{\scriptsize$\pm$1} \\
GCIQL~\cite{park2025ogbench} & 9\,{\scriptsize$\pm$1} & 8\,{\scriptsize$\pm$3} & 9\,{\scriptsize$\pm$1} & 3\,{\scriptsize$\pm$1} & 3\,{\scriptsize$\pm$1} \\
HILP~\cite{park2024foundation} & 12\,{\scriptsize$\pm$0} & 13\,{\scriptsize$\pm$4} & 16\,{\scriptsize$\pm$3} & 9\,{\scriptsize$\pm$1} & 10\,{\scriptsize$\pm$6} \\
\midrule
\rowcolor{oursrow}\textbf{Graph Anchors (ours)} & \textbf{62\,{\scriptsize$\pm$6}}$^{\ast}$ & \textbf{63\,{\scriptsize$\pm$7}}$^{\ast}$ & \textbf{73\,{\scriptsize$\pm$4}}$^{\ast}$ & \textbf{87\,{\scriptsize$\pm$1}}$^{\ast}$ & \textbf{66\,{\scriptsize$\pm$6}}$^{\ast}$ \\


==> tables/cmp_pmm_head.tex <==
PointMaze-M & $d{=}50$ & $d{=}100$ & $d{=}150$ & $d{=}200$ & stitched \\


==> tables/cmp_pmm_rows.tex <==
LeWM~\cite{maes2026leworldmodel} & 50\,{\scriptsize$\pm$12} & 25\,{\scriptsize$\pm$4} & 13\,{\scriptsize$\pm$3} & 13\,{\scriptsize$\pm$2} & 39\,{\scriptsize$\pm$10} \\
LeWM + min-over-plan & 70\,{\scriptsize$\pm$5} & 33\,{\scriptsize$\pm$6} & 17\,{\scriptsize$\pm$4} & 12\,{\scriptsize$\pm$5} & 41\,{\scriptsize$\pm$4} \\
\midrule
GCIVL~\cite{park2025ogbench} & 30$^\dagger$ & 4$^\dagger$ & 2$^\dagger$ & 0$^\dagger$ & 16\,{\scriptsize$\pm$0} \\
GCIQL~\cite{park2025ogbench} & 34\,{\scriptsize$\pm$5} & 4\,{\scriptsize$\pm$2} & 0\,{\scriptsize$\pm$0} & 1\,{\scriptsize$\pm$1} & 12\,{\scriptsize$\pm$3} \\
HILP~\cite{park2024foundation} & 32\,{\scriptsize$\pm$4} & 3\,{\scriptsize$\pm$2} & 1\,{\scriptsize$\pm$1} & 1\,{\scriptsize$\pm$1} & 18\,{\scriptsize$\pm$0} \\
\midrule
\rowcolor{oursrow}\textbf{Graph Anchors (ours)} & \textbf{91\,{\scriptsize$\pm$2}}$^{\ast}$ & \textbf{89\,{\scriptsize$\pm$4}}$^{\ast}$ & \textbf{88\,{\scriptsize$\pm$6}}$^{\ast}$ & \textbf{85\,{\scriptsize$\pm$6}}$^{\ast}$ & \textbf{95\,{\scriptsize$\pm$4}}$^{\ast}$ \\


==> tables/cmp_pusht_head.tex <==
Push-T & $d{=}25$ & $d{=}50$ & $d{=}75$ & $d{=}100$ & $d{=}150$ \\


==> tables/cmp_pusht_rows.tex <==
LeWM~\cite{maes2026leworldmodel} & 89\,{\scriptsize$\pm$1} & 41\,{\scriptsize$\pm$13} & 21\,{\scriptsize$\pm$4} & 17\,{\scriptsize$\pm$1} & 5\,{\scriptsize$\pm$4} \\
LeWM + min-over-plan & \textbf{91\,{\scriptsize$\pm$3}} & 55\,{\scriptsize$\pm$10} & 33\,{\scriptsize$\pm$7} & 17\,{\scriptsize$\pm$7} & 9\,{\scriptsize$\pm$1} \\
\midrule
GCIVL~\cite{park2025ogbench} & 2\,{\scriptsize$\pm$3} & 2\,{\scriptsize$\pm$0} & 0\,{\scriptsize$\pm$0} & 0\,{\scriptsize$\pm$0} & 0\,{\scriptsize$\pm$0} \\
GCIQL~\cite{park2025ogbench} & 0\,{\scriptsize$\pm$0} & 0\,{\scriptsize$\pm$0} & 0\,{\scriptsize$\pm$0} & 0\,{\scriptsize$\pm$0} & 0\,{\scriptsize$\pm$0} \\
HILP~\cite{park2024foundation} & 4\,{\scriptsize$\pm$3} & 0\,{\scriptsize$\pm$0} & 0\,{\scriptsize$\pm$0} & 0\,{\scriptsize$\pm$0} & 0\,{\scriptsize$\pm$0} \\
\midrule
\rowcolor{oursrow}\textbf{Graph Anchors (ours)} & 82\,{\scriptsize$\pm$6} & \textbf{65\,{\scriptsize$\pm$1}} & \textbf{50\,{\scriptsize$\pm$0}} & \textbf{40\,{\scriptsize$\pm$3}} & \textbf{30\,{\scriptsize$\pm$3}} \\


==> tables/cmp_tworoom_head.tex <==
Two-Room & $d{=}25$ & $d{=}50$ & $d{=}75$ & stitched \\


==> tables/cmp_tworoom_rows.tex <==
LeWM~\cite{maes2026leworldmodel} & 88\,{\scriptsize$\pm$4} & 54\,{\scriptsize$\pm$5} & 31\,{\scriptsize$\pm$3} & 61\,{\scriptsize$\pm$6} \\
LeWM + min-over-plan & \textbf{99\,{\scriptsize$\pm$1}} & 81\,{\scriptsize$\pm$5} & 62\,{\scriptsize$\pm$10} & 82\,{\scriptsize$\pm$3} \\
\midrule
GCIVL~\cite{park2025ogbench} & \textbf{99\,{\scriptsize$\pm$2}} & 90\,{\scriptsize$\pm$0} & 81\,{\scriptsize$\pm$2} & 86\,{\scriptsize$\pm$6} \\
GCIQL~\cite{park2025ogbench} & 61\,{\scriptsize$\pm$1} & 51\,{\scriptsize$\pm$11} & 37\,{\scriptsize$\pm$4} & 46\,{\scriptsize$\pm$0} \\
HILP~\cite{park2024foundation} & 98\,{\scriptsize$\pm$0} & \textbf{95\,{\scriptsize$\pm$1}} & 87\,{\scriptsize$\pm$3} & 89\,{\scriptsize$\pm$1} \\
\midrule
\rowcolor{oursrow}\textbf{Graph Anchors (ours)} & 96\,{\scriptsize$\pm$4} & 93\,{\scriptsize$\pm$1}$^{\ast}$ & \textbf{93\,{\scriptsize$\pm$1}}$^{\ast}$ & \textbf{99\,{\scriptsize$\pm$1}}$^{\ast}$ \\


==> tables/compare_rows.tex <==
\textbf{Push-T} & $d{=}25$ & $d{=}50$ & $d{=}75$ & $d{=}100$ & $d{=}150$ &  \\
\quad LeWM planner~\cite{maes2026leworldmodel} & 88 & 41 & 21 & 17 & 5 & -- \\
\quad LeWM + min-over-plan & \textbf{94} & 55 & 33 & 17 & 9 & -- \\
\quad GCBC~\cite{park2025ogbench} & -- & 16 & 8 & 11 & 5 & -- \\
\quad GCIVL~\cite{park2025ogbench} & -- & 2 & 0 & 0 & 0 & -- \\
\quad GCIQL~\cite{park2025ogbench} & -- & 0 & 0 & 0 & 0 & -- \\
\quad HILP~\cite{park2024foundation} & -- & 0 & 0 & 0 & 0 & -- \\
\rowcolor{pactrow}\quad \textbf{Graph anchors (ours)} & -- & \textbf{65} & \textbf{50} & \textbf{40} & \textbf{30} & -- \\
\midrule
\textbf{Two-Room} & $d{=}25$ & $d{=}50$ & $d{=}75$ &  &  & stitched \\
\quad LeWM planner~\cite{maes2026leworldmodel} & 88 & 54 & 31 &  &  & 61 \\
\quad LeWM + min-over-plan & 99 & 81 & 62 &  &  & 82 \\
\quad DINO-WM~\cite{zhou2024dino}$^\ddagger$ & -- & 90 & 70 &  &  & 95 \\
\quad GCBC~\cite{park2025ogbench} & \textbf{100} & \textbf{98} & \textbf{100} &  &  & \textbf{99} \\
\quad GCIVL~\cite{park2025ogbench} & 99 & 90 & 81 &  &  & 86 \\
\quad GCIQL~\cite{park2025ogbench} & 61 & 51 & 37 &  &  & 46 \\
\quad HILP~\cite{park2024foundation} & 98 & 95 & 87 &  &  & 89 \\
\rowcolor{pactrow}\quad \textbf{Graph anchors (ours)} & 96 & 93 & 93 &  &  & 99 \\
\midrule
\textbf{PointMaze-M} & $d{=}50$ & $d{=}100$ & $d{=}150$ & $d{=}200$ &  & stitched \\
\quad LeWM planner~\cite{maes2026leworldmodel} & 50 & 25 & 13 & 13 &  & 39 \\
\quad LeWM + min-over-plan & 70 & 33 & 17 & 12 &  & 41 \\
\quad DINO-WM~\cite{zhou2024dino}$^\ddagger$ & -- & 70 & -- & 15 &  & 35 \\
\quad GCBC~\cite{park2025ogbench} & \textbf{93} & 83 & 54 & 51 &  & 51 \\
\quad GCIVL~\cite{park2025ogbench} & 30 & 4 & 2 & 0 &  & 16 \\
\quad GCIQL~\cite{park2025ogbench} & 34 & 4 & 0 & 1 &  & 12 \\
\quad HILP~\cite{park2024foundation} & 32 & 3 & 1 & 1 &  & 18 \\
\rowcolor{pactrow}\quad \textbf{Graph anchors (ours)} & 91 & \textbf{89} & \textbf{88} & \textbf{85} &  & \textbf{95} \\
\midrule
\textbf{PointMaze-L} & $d{=}50$ & $d{=}100$ & $d{=}200$ & $d{=}400$ &  & stitched \\
\quad LeWM planner~\cite{maes2026leworldmodel} & 14 & 15 & 13 & 8 &  & 5 \\
\quad LeWM + min-over-plan & 44 & 28 & 23 & 26 &  & 17 \\
\quad DINO-WM~\cite{zhou2024dino}$^\ddagger$ & -- & -- & \textbf{95} & \textbf{100} &  & \textbf{100} \\
\quad GCBC~\cite{park2025ogbench} & 33 & 25 & 18 & 18 &  & 17 \\
\quad GCIVL~\cite{park2025ogbench} & 9 & 8 & 9 & 1 &  & 3 \\
\quad GCIQL~\cite{park2025ogbench} & 9 & 8 & 9 & 3 &  & 3 \\
\quad HILP~\cite{park2024foundation} & 12 & 13 & 16 & 9 &  & 10 \\
\rowcolor{pactrow}\quad \textbf{Graph anchors (ours)} & \textbf{62} & \textbf{63} & 73 & 87 &  & 66 \\


==> tables/contemp_apoff_rows.tex <==
PointMaze-M, $d{=}100$ & 47 & 59 & 95 & 91 & 74 & 53 & 15 & 89 \\
PointMaze-M, $d{=}200$ & 29 & 29 & 54 & 80 & 70 & 45 & 11 & 85 \\
Two-Room, $d{=}75$ & 36 & 82 & 98 & 97 & 98 & 96 & 2 & 93 \\
PointMaze-L, $d{=}200$ & -- & 17 & -- & 16 & -- & 17 & -- & 73 \\
PointMaze-L, $d{=}400$ & -- & 11 & -- & 12 & -- & 14 & -- & 87 \\


==> tables/contemp_apoff_rows_clean.tex <==
PointMaze-M, $d{=}100$ & 47 & 59 & 95 & 91 & 74 & 53 & 15 & 89 \\
PointMaze-M, $d{=}200$ & 29 & 29 & 54 & 80 & 70 & 45 & 11 & 85 \\
Two-Room, $d{=}75$ & 36 & 82 & 98 & 97 & 98 & 96 & 2 & 93 \\
Push-T, $d{=}150$ & -- & 16 & -- & 65 & -- & 2 & 0 & 71$^c$ \\


==> tables/contemp_sweep_rows.tex <==
PointMaze-Medium, $d{=}200$ & 82 & 96 & 92 & \textbf{98} & 96 & 90 \\
Two-Room, $d{=}75$ & 22 & \textbf{100} & 96 & 72 & 42 & 30 \\
Push-T, $d{=}75$ & 24 & 36 & 50 & \textbf{58} & \textbf{58} & 56 \\
Push-T, $d{=}150$ & -- & 8 & -- & 24 & \textbf{28} & -- \\


==> tables/drift_main_rows.tex <==
PointMaze-M, $d{=}200$ & 48\,{\scriptsize[46,\,50]} & 47\,{\scriptsize[45,\,49]} & \textbf{72}\,{\scriptsize[70,\,75]} \\
Two-Room, $d{=}75$ & 33\,{\scriptsize[29,\,37]} & 46\,{\scriptsize[41,\,51]} & \textbf{74}\,{\scriptsize[71,\,78]} \\
Push-T, $d{=}150$ & 31\,{\scriptsize[28,\,34]} & 37\,{\scriptsize[34,\,40]} & \textbf{53}\,{\scriptsize[50,\,56]} \\


==> tables/drift_t8_rows.tex <==
\multicolumn{6}{l}{\emph{Two-Room}, $d{=}75$}\\
LeWM & 32 & 705 & 33 [29, 37] & $-$0.08 & --\\
LeWM + min-over-plan & 61 & 533 & 46 [41, 51] & $-$0.60 & --\\
Graph Anchors & 94 & 474 & 74 [71, 78] & $-$1.54 & --\\
\multicolumn{6}{l}{\emph{Push-T}, $d{=}150$}\\
LeWM & 4 & 1106 & 31 [28, 34] & $-$0.03 & 28 [24, 31]\\
LeWM + min-over-plan & 6 & 1050 & 37 [34, 40] & $-$0.14 & 31 [28, 35]\\
Graph Anchors & 31 & 979 & 53 [50, 56] & $-$0.67 & 46 [41, 50]\\
Graph Anchors, $\lambda{=}3$ & 46 & 897 & 54 [51, 58] & $-$0.77 & 47 [43, 51]\\


==> tables/drift_t8_rows_clean.tex <==
\multicolumn{5}{l}{\emph{Two-Room}, $d{=}75$}\\
LeWM & 32 & 705 & 33 [29, 37] & $-$0.08 \\
LeWM + min-over-plan & 61 & 533 & 46 [41, 51] & $-$0.60 \\
Graph Anchors & 94 & 474 & 74 [71, 78] & $-$1.54 \\
\multicolumn{5}{l}{\emph{Push-T}, $d{=}150$}\\
LeWM & 4 & 1106 & 31 [28, 34] & $-$0.03 \\
LeWM + min-over-plan & 6 & 1050 & 37 [34, 40] & $-$0.14 \\
Graph Anchors & 31 & 979 & 53 [50, 56] & $-$0.67 \\
Graph Anchors, $\lambda{=}3$ & 46 & 897 & 54 [51, 58] & $-$0.77 \\


==> tables/graphpol_rows.tex <==
GCBC + graph waypoints & 84 & 70 & 39 & 21 & 41 & 17 & 15 & 10 & 6 & 4\\
GCIVL + graph waypoints & 34 & 8 & 3 & 0 & 18 & 8 & 7 & 9 & 2 & 1\\
HILP + graph waypoints & 31 & 3 & 1 & 0 & 18 & 8 & 9 & 8 & 7 & 4\\
GAS-style (HILP) & 31 & 3 & 1 & 0 & 18 & 9 & 10 & 10 & 10 & 8\\
\midrule
GCBC, no graph & \textbf{93} & 83 & 54 & 51 & 51 & 33 & 25 & 18 & 18 & 17\\
HILP, no graph & 32 & 3 & 1 & 1 & 18 & 12 & 13 & 16 & 9 & 10\\
\midrule
Graph Anchors (ours) & 91 & \textbf{89} & \textbf{88} & \textbf{85} & \textbf{95} & \textbf{62} & \textbf{63} & \textbf{73} & \textbf{87} & \textbf{66}\\


==> tables/main_cmp_rows.tex <==
LeWM planner~\cite{maes2026leworldmodel} & 17 & 5 & 31 & 61 & 13 & 39 & 8 & 5 & 70 & 60 \\
LeWM + min-over-plan & 17 & 9 & 62 & 82 & 12 & 41 & 26 & 17 & 73 & 77 \\
PLDM~\cite{sobal2026learning} & 0 & 0 & 50 & 81 & 3 & 28 & 1 & 2 & 17 & 15 \\
DINO-WM~\cite{zhou2024dino}$^\ddagger$ & -- & -- & 70 & 95 & 15 & 35 & \textbf{100} & \textbf{100} & -- & -- \\
\midrule
GCBC~\cite{park2025ogbench} & 11 & 5 & \textbf{100} & \textbf{99} & 51 & 51 & 18 & 17 & 0 & 0 \\
GCIVL~\cite{park2025ogbench} & 0 & 0 & 81 & 86 & 0 & 16 & 1 & 3 & 0 & 0 \\
GCIQL~\cite{park2025ogbench} & 0 & 0 & 37 & 46 & 1 & 12 & 3 & 3 & 0 & 0 \\
HILP~\cite{park2024foundation} & 0 & 0 & 87 & 89 & 1 & 18 & 9 & 10 & 0 & 0 \\
\midrule
\rowcolor{pactrow}\textbf{Graph anchors (ours)} & 40 & 30 & 93 & 99 & 85 & \textbf{95} & 87 & 66 & 66 & 68 \\
\quad + switch cost $\lambda{=}3$ & \textbf{56} & \textbf{48} & 83 & 98 & 77 & 84 & 92 & 66 & 78 & 73 \\
\quad + goal handoff & 45 & 35 & 87 & 96 & \textbf{86} & 86 & 86 & 61 & \textbf{86} & \textbf{80} \\


==> tables/main_labels.tex <==
% generated by figs/scripts/export_labels.py from main.aux; do not edit
\newlabel{sec:intro}{{1}{1}{}{}{}}
\newlabel{sec:intro@cref}{{[section][1][]1}{[1][1][]1}{}{}{}}
\newlabel{fig:teaser}{{1}{1}{}{}{}}
\newlabel{fig:teaser@cref}{{[figure][1][]1}{[1][1][]1}{}{}{}}
\newlabel{sec:related}{{2}{2}{}{}{}}
\newlabel{sec:related@cref}{{[section][2][]2}{[1][2][]2}{}{}{}}
\newlabel{sec:prelim}{{3}{2}{}{}{}}
\newlabel{sec:prelim@cref}{{[section][3][]3}{[1][2][]2}{}{}{}}
\newlabel{eq:wm}{{1}{2}{}{}{}}
\newlabel{eq:wm@cref}{{[equation][1][]1}{[1][2][]2}{}{}{}}
\newlabel{eq:plan}{{2}{2}{}{}{}}
\newlabel{eq:plan@cref}{{[equation][2][]2}{[1][2][]2}{}{}{}}
\newlabel{sec:method}{{4}{2}{}{}{}}
\newlabel{sec:method@cref}{{[section][4][]4}{[1][2][]2}{}{}{}}
\newlabel{sec:problem}{{4.1}{3}{}{}{}}
\newlabel{sec:problem@cref}{{[subsection][1][4]4.1}{[1][3][]3}{}{}{}}
\newlabel{sec:diagnosis}{{4.1}{3}{}{}{}}
\newlabel{sec:diagnosis@cref}{{[subsection][1][4]4.1}{[1][3][]3}{}{}{}}
\newlabel{eq:rho}{{3}{3}{}{}{}}
\newlabel{eq:rho@cref}{{[equation][3][]3}{[1][3][]3}{}{}{}}
\newlabel{fig:diagnosis}{{2}{3}{}{}{}}
\newlabel{fig:diagnosis@cref}{{[figure][2][]2}{[1][3][]3}{}{}{}}
\newlabel{sec:graph}{{4.2}{3}{}{}{}}
\newlabel{sec:graph@cref}{{[subsection][2][4]4.2}{[1][3][]3}{}{}{}}
\newlabel{fig:method}{{3}{4}{}{}{}}
\newlabel{fig:method@cref}{{[figure][3][]3}{[1][3][]4}{}{}{}}
\newlabel{eq:edges}{{4}{4}{}{}{}}
\newlabel{eq:edges@cref}{{[equation][4][]4}{[1][3][]4}{}{}{}}
\newlabel{fig:whygraph}{{4}{4}{}{}{}}
\newlabel{fig:whygraph@cref}{{[figure][4][]4}{[1][4][]4}{}{}{}}
\newlabel{sec:anchor}{{4.3}{4}{}{}{}}
\newlabel{sec:anchor@cref}{{[subsection][3][4]4.3}{[1][4][]4}{}{}{}}
\newlabel{eq:anchor}{{5}{4}{}{}{}}
\newlabel{eq:anchor@cref}{{[equation][5][]5}{[1][4][]4}{}{}{}}
\newlabel{eq:transfer}{{6}{5}{}{}{}}
\newlabel{eq:transfer@cref}{{[equation][6][]6}{[1][5][]5}{}{}{}}
\newlabel{sec:switch}{{4.4}{5}{}{}{}}
\newlabel{sec:switch@cref}{{[subsection][4][4]4.4}{[1][5][]5}{}{}{}}
\newlabel{eq:switch}{{7}{5}{}{}{}}
\newlabel{eq:switch@cref}{{[equation][7][]7}{[1][5][]5}{}{}{}}
\newlabel{sec:search}{{4.5}{5}{}{}{}}
\newlabel{sec:search@cref}{{[subsection][5][4]4.5}{[1][5][]5}{}{}{}}
\newlabel{eq:cost}{{8}{5}{}{}{}}
\newlabel{eq:cost@cref}{{[equation][8][]8}{[1][5][]5}{}{}{}}
\newlabel{alg:ga}{{1}{5}{}{}{}}
\newlabel{alg:ga@cref}{{[algorithm][1][]1}{[1][5][]5}{}{}{}}
\newlabel{sec:objective}{{4.6}{5}{}{}{}}
\newlabel{sec:objective@cref}{{[subsection][6][4]4.6}{[1][5][]5}{}{}{}}
\newlabel{eq:overall}{{9}{5}{}{}{}}
\newlabel{eq:overall@cref}{{[equation][9][]9}{[1][5][]5}{}{}{}}
\newlabel{sec:experiments}{{5}{5}{}{}{}}
\newlabel{sec:experiments@cref}{{[section][5][]5}{[1][5][]5}{}{}{}}
\newlabel{tab:main}{{1}{6}{}{}{}}
\newlabel{tab:main@cref}{{[table][1][]1}{[1][5][]6}{}{}{}}
\newlabel{fig:frames}{{5}{6}{}{}{}}
\newlabel{fig:frames@cref}{{[figure][5][]5}{[1][5][]6}{}{}{}}
\newlabel{sec:p1}{{5.1}{6}{}{}{}}
\newlabel{sec:p1@cref}{{[subsection][1][5]5.1}{[1][6][]6}{}{}{}}
\newlabel{sec:compare}{{5.1}{6}{}{}{}}
\newlabel{sec:compare@cref}{{[subsection][1][5]5.1}{[1][6][]6}{}{}{}}
\newlabel{fig:results}{{6}{7}{}{}{}}
\newlabel{fig:results@cref}{{[figure][6][]6}{[1][6][]7}{}{}{}}
\newlabel{fig:ablations}{{7}{7}{}{}{}}
\newlabel{fig:ablations@cref}{{[figure][7][]7}{[1][6][]7}{}{}{}}
\newlabel{fig:contact}{{7}{7}{}{}{}}
\newlabel{fig:contact@cref}{{[figure][7][]7}{[1][6][]7}{}{}{}}
\newlabel{sec:contact}{{5.2}{7}{}{}{}}
\newlabel{sec:contact@cref}{{[subsection][2][5]5.2}{[1][7][]7}{}{}{}}
\newlabel{sec:ablation}{{5.3}{7}{}{}{}}
\newlabel{sec:ablation@cref}{{[subsection][3][5]5.3}{[1][7][]7}{}{}{}}
\newlabel{sec:design}{{5.4}{7}{}{}{}}
\newlabel{sec:design@cref}{{[subsection][4][5]5.4}{[1][7][]7}{}{}{}}
\newlabel{fig:robustbars}{{8}{8}{}{}{}}
\newlabel{fig:robustbars@cref}{{[figure][8][]8}{[1][8][]8}{}{}{}}
\newlabel{sec:where}{{5.5}{8}{}{}{}}
\newlabel{sec:where@cref}{{[subsection][5][5]5.5}{[1][8][]8}{}{}{}}
\newlabel{sec:negative}{{5.5}{8}{}{}{}}
\newlabel{sec:negative@cref}{{[subsection][5][5]5.5}{[1][8][]8}{}{}{}}
\newlabel{sec:beyond}{{5.5}{8}{}{}{}}
\newlabel{sec:beyond@cref}{{[subsection][5][5]5.5}{[1][8][]8}{}{}{}}
\newlabel{fig:predict}{{9}{8}{}{}{}}
\newlabel{fig:predict@cref}{{[figure][9][]9}{[1][8][]8}{}{}{}}
\newlabel{tab:where}{{2}{8}{}{}{}}
\newlabel{tab:where@cref}{{[table][2][]2}{[1][8][]8}{}{}{}}
\newlabel{sec:conclusion}{{6}{8}{}{}{}}
\newlabel{sec:conclusion@cref}{{[section][6][]6}{[1][8][]8}{}{}{}}


==> tables/main_lewm_rows.tex <==
\textbf{Push-T} & $d{=}25$ & $d{=}50$ & $d{=}75$ & $d{=}100$ & $d{=}150$ &  \\
\quad LeWM planner~\cite{maes2026leworldmodel} & 88 & 41 & 21 & 17 & 5 & -- \\
\quad LeWM + min-over-plan & \textbf{94} & 55 & 33 & 17 & 9 & -- \\
\rowcolor{pactrow}\quad \textbf{Graph anchors (ours)} & -- & \textbf{65} & \textbf{50} & \textbf{40} & \textbf{30} & -- \\
\midrule
\textbf{Two-Room} & $d{=}25$ & $d{=}50$ & $d{=}75$ &  &  & stitched \\
\quad LeWM planner~\cite{maes2026leworldmodel} & 88 & 54 & 31 &  &  & 61 \\
\quad LeWM + min-over-plan & \textbf{99} & 81 & 62 &  &  & 82 \\
\rowcolor{pactrow}\quad \textbf{Graph anchors (ours)} & 96 & \textbf{93} & \textbf{93} &  &  & \textbf{99} \\
\midrule
\textbf{PointMaze-M} & $d{=}50$ & $d{=}100$ & $d{=}150$ & $d{=}200$ &  & stitched \\
\quad LeWM planner~\cite{maes2026leworldmodel} & 50 & 25 & 13 & 13 &  & 39 \\
\quad LeWM + min-over-plan & 70 & 33 & 17 & 12 &  & 41 \\
\rowcolor{pactrow}\quad \textbf{Graph anchors (ours)} & \textbf{91} & \textbf{89} & \textbf{88} & \textbf{85} &  & \textbf{95} \\
\midrule
\textbf{PointMaze-L} & $d{=}50$ & $d{=}100$ & $d{=}200$ & $d{=}400$ &  & stitched \\
\quad LeWM planner~\cite{maes2026leworldmodel} & 14 & 15 & 13 & 8 &  & 5 \\
\quad LeWM + min-over-plan & 44 & 28 & 23 & 26 &  & 17 \\
\rowcolor{pactrow}\quad \textbf{Graph anchors (ours)} & \textbf{62} & \textbf{63} & \textbf{73} & \textbf{87} &  & \textbf{66} \\


==> tables/main_rows.tex <==
\textbf{Push-T} & $d{=}25$ & $d{=}50$ & $d{=}75$ & $d{=}100$ & $d{=}150$ \\
\quad LeWM planner & 88 & 41 & 21 & 17 & 5 \\
\quad LeWM + min-over-plan & \textbf{94} & 55 & 33 & 17 & 9 \\
\rowcolor{pactrow}\quad Graph anchors (ours) & -- & \textbf{65} & \textbf{50} & \textbf{40} & \textbf{30} \\
\midrule
\textbf{Two-Room} & $d{=}25$ & $d{=}50$ & $d{=}75$ &  &  \\
\quad LeWM planner & 86 & 51 & 30 &  &  \\
\quad LeWM + min-over-plan & \textbf{98} & 81 & 59 &  &  \\
\rowcolor{pactrow}\quad Graph anchors (ours) & 94 & \textbf{93} & \textbf{93} &  &  \\
\midrule
\textbf{PointMaze-M} & $d{=}50$ & $d{=}100$ & $d{=}150$ & $d{=}200$ &  \\
\quad LeWM planner & 44 & 23 & 11 & 14 &  \\
\quad LeWM + min-over-plan & 67 & 35 & 16 & 10 &  \\
\rowcolor{pactrow}\quad Graph anchors (ours) & \textbf{90} & \textbf{88} & \textbf{91} & \textbf{86} &  \\
\midrule[0.8pt]
\textbf{OGBench-Cube} & $d{=}25$ & $d{=}50$ & $d{=}100$ & $d{=}150$ &  \\
\quad LeWM planner & 70 & 64 & 50 & 20 &  \\
\quad LeWM + min-over-plan & 68 & 60 & 56 & 20 &  \\
\rowcolor{pactrow}\quad Graph anchors (ours) & 70 & 56 & 60 & 20 &  \\
\midrule
\textbf{Reacher} & $d{=}25$ & $d{=}50$ & $d{=}100$ & $d{=}150$ &  \\
\quad LeWM planner & 60 & 74 & 62 & 66 &  \\
\quad LeWM + min-over-plan & 82 & 80 & 78 & 74 &  \\
\rowcolor{pactrow}\quad Graph anchors (ours) & 60 & 60 & 64 & 64 &  \\


==> tables/mw_rows.tex <==
Released latent cost~\cite{terver2025drives} & 0 & 0 & 0 & 0 & 0 & 0 & 0.0 & 100 & 96 \\
TEMPO temporal distance~\cite{moukheiber2026long} & 0 & 0 & 0 & 0 & 0 & 0 & 0.0 & 100 & 42 \\
State head (privileged labels) & 0 & 0 & 0 & 67 & 0 & 0 & 11.1 & 100 & 58 \\
Image-only reach-then-change & 25 & 0 & 8 & 0 & 0 & 0 & 5.6 & 83 & 67 \\
Progress head, demonstrations only & 0 & 25 & 0 & 8 & 0 & 17 & 8.3 & 100 & -- \\
\midrule
Cost trained on planner states, one round & 25 & 58 & \textbf{83} & \textbf{92} & 17 & 58 & 55.6 & 100 & 92 \\
\rowcolor{pactrow}\textbf{Cost trained on planner states, two rounds} & \textbf{83} & \textbf{83} & 25 & \textbf{92} & \textbf{33} & \textbf{92} & \textbf{68.1} & 100 & 83 \\
\midrule
\textit{Oracle: true object state} & 0 & 92 & 83 & 83 & 33 & -- & -- & 100 & -- \\


==> tables/mwdemo_rows.tex <==
\textit{Demonstration target, 20 steps ahead (privileged)} & 100 & 50 & 100 & 100 & 92 & 100 & 90.3 & -- & -- \\


==> tables/mwdemo_rows_clean.tex <==
% demonstration row moved to the text (controls not run)


==> tables/numbers.tex <==
% generated by figs/scripts/make_tables.py -- do not edit
\makeatletter
\newcommand{\numH}[1]{\csname numH@#1\endcsname}
\newcommand{\diagA}[2]{\csname diagA@#1@#2\endcsname}
\newcommand{\hops}[2]{\csname hops@#1@#2\endcsname}
\newcommand{\cubeNT}[1]{\csname cubeNT@#1\endcsname}
\expandafter\def\csname numH@10\endcsname{98\%}
\expandafter\def\csname numH@20\endcsname{92\%}
\expandafter\def\csname numH@30\endcsname{81\%}
\expandafter\def\csname numH@40\endcsname{56\%}
\expandafter\def\csname numH@50\endcsname{36\%}
\expandafter\def\csname numH@60\endcsname{29\%}
\expandafter\def\csname diagA@pusht@1\endcsname{0.91}
\expandafter\def\csname diagA@pusht@2\endcsname{0.85}
\expandafter\def\csname diagA@pusht@3\endcsname{0.78}
\expandafter\def\csname diagA@pusht@4\endcsname{0.74}
\expandafter\def\csname diagA@pusht@5\endcsname{0.74}
\expandafter\def\csname diagA@pusht@6\endcsname{0.74}
\expandafter\def\csname diagA@pusht@7\endcsname{0.73}
\expandafter\def\csname diagA@pusht@8\endcsname{0.72}
\expandafter\def\csname diagA@pusht@9\endcsname{0.68}
\expandafter\def\csname diagA@pusht@10\endcsname{0.68}
\expandafter\def\csname diagA@pusht@11\endcsname{0.65}
\expandafter\def\csname diagA@pusht@12\endcsname{0.62}
\expandafter\def\csname diagA@pusht@13\endcsname{0.61}
\expandafter\def\csname diagA@pusht@14\endcsname{0.58}
\expandafter\def\csname diagA@pusht@15\endcsname{0.56}
\expandafter\def\csname diagA@pusht@16\endcsname{0.56}
\expandafter\def\csname diagA@pusht@17\endcsname{0.55}
\expandafter\def\csname diagA@pusht@18\endcsname{0.56}
\expandafter\def\csname diagA@pusht@19\endcsname{0.55}
\expandafter\def\csname diagA@pusht@20\endcsname{0.55}
\expandafter\def\csname diagA@pusht@21\endcsname{0.53}
\expandafter\def\csname diagA@pusht@22\endcsname{0.52}
\expandafter\def\csname diagA@pusht@23\endcsname{0.52}
\expandafter\def\csname diagA@pusht@24\endcsname{0.51}
\expandafter\def\csname diagA@pusht@25\endcsname{0.49}
\expandafter\def\csname diagA@pusht@26\endcsname{0.48}
\expandafter\def\csname diagA@pusht@27\endcsname{0.43}
\expandafter\def\csname diagA@pusht@28\endcsname{0.40}
\expandafter\def\csname diagA@pusht@29\endcsname{0.43}
\expandafter\def\csname diagA@pusht@30\endcsname{0.38}
\expandafter\def\csname diagA@pusht@31\endcsname{0.37}
\expandafter\def\csname diagA@pusht@32\endcsname{0.34}
\expandafter\def\csname diagA@pusht@33\endcsname{0.38}
\expandafter\def\csname diagA@pusht@34\endcsname{0.44}
\expandafter\def\csname diagA@pusht@35\endcsname{0.39}
\expandafter\def\csname diagA@pusht@36\endcsname{0.37}
\expandafter\def\csname diagA@pusht@37\endcsname{0.47}
\expandafter\def\csname diagA@pusht@38\endcsname{0.33}
\expandafter\def\csname diagA@pusht@39\endcsname{0.62}
\expandafter\def\csname diagA@pusht@40\endcsname{0.67}
\expandafter\def\csname hops@pusht@25\endcsname{5}
\expandafter\def\csname hops@pusht@50\endcsname{10}
\expandafter\def\csname hops@pusht@75\endcsname{14}
\expandafter\def\csname hops@pusht@100\endcsname{16}
\expandafter\def\csname hops@pusht@150\endcsname{18}
\expandafter\def\csname hops@pusht@200\endcsname{20}
\expandafter\def\csname diagA@tworoom@1\endcsname{0.99}
\expandafter\def\csname diagA@tworoom@2\endcsname{0.85}
\expandafter\def\csname diagA@tworoom@3\endcsname{0.61}
\expandafter\def\csname diagA@tworoom@4\endcsname{0.55}
\expandafter\def\csname diagA@tworoom@5\endcsname{0.54}
\expandafter\def\csname diagA@tworoom@6\endcsname{0.50}
\expandafter\def\csname diagA@tworoom@7\endcsname{0.51}
\expandafter\def\csname diagA@tworoom@8\endcsname{0.50}
\expandafter\def\csname diagA@tworoom@9\endcsname{0.50}
\expandafter\def\csname diagA@tworoom@10\endcsname{0.51}
\expandafter\def\csname diagA@tworoom@11\endcsname{0.51}
\expandafter\def\csname diagA@tworoom@12\endcsname{0.51}
\expandafter\def\csname diagA@tworoom@13\endcsname{0.51}
\expandafter\def\csname diagA@tworoom@14\endcsname{0.47}
\expandafter\def\csname diagA@tworoom@15\endcsname{0.45}
\expandafter\def\csname diagA@tworoom@16\endcsname{0.45}
\expandafter\def\csname diagA@tworoom@17\endcsname{0.44}
\expandafter\def\csname diagA@tworoom@18\endcsname{0.44}
\expandafter\def\csname diagA@tworoom@19\endcsname{0.44}
\expandafter\def\csname diagA@tworoom@20\endcsname{0.45}
\expandafter\def\csname diagA@tworoom@21\endcsname{0.42}
\expandafter\def\csname diagA@tworoom@22\endcsname{0.45}
\expandafter\def\csname diagA@tworoom@23\endcsname{0.46}
\expandafter\def\csname diagA@tworoom@24\endcsname{0.46}
\expandafter\def\csname diagA@tworoom@25\endcsname{0.46}
\expandafter\def\csname diagA@tworoom@26\endcsname{0.40}
\expandafter\def\csname diagA@tworoom@27\endcsname{0.45}
\expandafter\def\csname diagA@tworoom@28\endcsname{0.43}
\expandafter\def\csname diagA@tworoom@29\endcsname{0.32}
\expandafter\def\csname diagA@tworoom@30\endcsname{0.30}
\expandafter\def\csname hops@tworoom@25\endcsname{5}
\expandafter\def\csname hops@tworoom@50\endcsname{9}
\expandafter\def\csname hops@tworoom@75\endcsname{11}
\expandafter\def\csname diagA@pmm@1\endcsname{0.99}
\expandafter\def\csname diagA@pmm@2\endcsname{0.83}
\expandafter\def\csname diagA@pmm@3\endcsname{0.65}
\expandafter\def\csname diagA@pmm@4\endcsname{0.61}
\expandafter\def\csname diagA@pmm@5\endcsname{0.59}
\expandafter\def\csname diagA@pmm@6\endcsname{0.59}
\expandafter\def\csname diagA@pmm@7\endcsname{0.58}
\expandafter\def\csname diagA@pmm@8\endcsname{0.59}
\expandafter\def\csname diagA@pmm@9\endcsname{0.55}
\expandafter\def\csname diagA@pmm@10\endcsname{0.51}
\expandafter\def\csname diagA@pmm@11\endcsname{0.48}
\expandafter\def\csname diagA@pmm@12\endcsname{0.46}
\expandafter\def\csname diagA@pmm@13\endcsname{0.45}
\expandafter\def\csname diagA@pmm@14\endcsname{0.46}
\expandafter\def\csname diagA@pmm@15\endcsname{0.48}
\expandafter\def\csname diagA@pmm@16\endcsname{0.49}
\expandafter\def\csname diagA@pmm@17\endcsname{0.52}
\expandafter\def\csname diagA@pmm@18\endcsname{0.53}
\expandafter\def\csname diagA@pmm@19\endcsname{0.51}
\expandafter\def\csname diagA@pmm@20\endcsname{0.50}
\expandafter\def\csname diagA@pmm@21\endcsname{0.50}
\expandafter\def\csname diagA@pmm@22\endcsname{0.50}
\expandafter\def\csname diagA@pmm@23\endcsname{0.49}
\expandafter\def\csname diagA@pmm@24\endcsname{0.50}
\expandafter\def\csname diagA@pmm@25\endcsname{0.50}
\expandafter\def\csname diagA@pmm@26\endcsname{0.51}
\expandafter\def\csname diagA@pmm@27\endcsname{0.50}
\expandafter\def\csname diagA@pmm@28\endcsname{0.51}
\expandafter\def\csname diagA@pmm@29\endcsname{0.51}
\expandafter\def\csname diagA@pmm@30\endcsname{0.51}
\expandafter\def\csname diagA@pmm@31\endcsname{0.50}
\expandafter\def\csname diagA@pmm@32\endcsname{0.52}
\expandafter\def\csname diagA@pmm@33\endcsname{0.50}
\expandafter\def\csname diagA@pmm@34\endcsname{0.51}
\expandafter\def\csname diagA@pmm@35\endcsname{0.52}
\expandafter\def\csname diagA@pmm@36\endcsname{0.51}
\expandafter\def\csname diagA@pmm@37\endcsname{0.51}
\expandafter\def\csname diagA@pmm@38\endcsname{0.51}
\expandafter\def\csname diagA@pmm@39\endcsname{0.51}
\expandafter\def\csname diagA@pmm@40\endcsname{0.49}
\expandafter\def\csname hops@pmm@25\endcsname{5}
\expandafter\def\csname hops@pmm@50\endcsname{10}
\expandafter\def\csname hops@pmm@75\endcsname{15}
\expandafter\def\csname hops@pmm@100\endcsname{20}
\expandafter\def\csname hops@pmm@150\endcsname{29}
\expandafter\def\csname hops@pmm@200\endcsname{34}
\expandafter\def\csname diagA@cube@1\endcsname{0.99}
\expandafter\def\csname diagA@cube@2\endcsname{0.92}
\expandafter\def\csname diagA@cube@3\endcsname{0.85}
\expandafter\def\csname diagA@cube@4\endcsname{0.82}
\expandafter\def\csname diagA@cube@5\endcsname{0.80}
\expandafter\def\csname diagA@cube@6\endcsname{0.77}
\expandafter\def\csname diagA@cube@7\endcsname{0.74}
\expandafter\def\csname diagA@cube@8\endcsname{0.69}
\expandafter\def\csname diagA@cube@9\endcsname{0.64}
\expandafter\def\csname diagA@cube@10\endcsname{0.60}
\expandafter\def\csname diagA@cube@11\endcsname{0.58}
\expandafter\def\csname diagA@cube@12\endcsname{0.57}
\expandafter\def\csname diagA@cube@13\endcsname{0.56}
\expandafter\def\csname diagA@cube@14\endcsname{0.57}
\expandafter\def\csname diagA@cube@15\endcsname{0.58}
\expandafter\def\csname diagA@cube@16\endcsname{0.57}
\expandafter\def\csname diagA@cube@17\endcsname{0.59}
\expandafter\def\csname diagA@cube@18\endcsname{0.61}
\expandafter\def\csname diagA@cube@19\endcsname{0.59}
\expandafter\def\csname diagA@cube@20\endcsname{0.57}
\expandafter\def\csname diagA@cube@21\endcsname{0.56}
\expandafter\def\csname diagA@cube@22\endcsname{0.49}
\expandafter\def\csname diagA@cube@23\endcsname{0.56}
\expandafter\def\csname hops@cube@25\endcsname{5}
\expandafter\def\csname hops@cube@50\endcsname{7}
\expandafter\def\csname hops@cube@75\endcsname{5}
\expandafter\def\csname hops@cube@100\endcsname{5}
\expandafter\def\csname hops@cube@150\endcsname{13}
\expandafter\def\csname diagA@reacher@1\endcsname{1.00}
\expandafter\def\csname diagA@reacher@2\endcsname{0.88}
\expandafter\def\csname diagA@reacher@3\endcsname{0.66}
\expandafter\def\csname diagA@reacher@4\endcsname{0.59}
\expandafter\def\csname diagA@reacher@5\endcsname{0.57}
\expandafter\def\csname diagA@reacher@6\endcsname{0.56}
\expandafter\def\csname diagA@reacher@7\endcsname{0.55}
\expandafter\def\csname diagA@reacher@8\endcsname{0.50}
\expandafter\def\csname diagA@reacher@9\endcsname{0.48}
\expandafter\def\csname diagA@reacher@10\endcsname{0.49}
\expandafter\def\csname diagA@reacher@11\endcsname{0.51}
\expandafter\def\csname diagA@reacher@12\endcsname{0.51}
\expandafter\def\csname diagA@reacher@13\endcsname{0.51}
\expandafter\def\csname diagA@reacher@14\endcsname{0.52}
\expandafter\def\csname diagA@reacher@15\endcsname{0.51}
\expandafter\def\csname diagA@reacher@16\endcsname{0.51}
\expandafter\def\csname diagA@reacher@17\endcsname{0.51}
\expandafter\def\csname diagA@reacher@18\endcsname{0.52}
\expandafter\def\csname diagA@reacher@19\endcsname{0.52}
\expandafter\def\csname diagA@reacher@20\endcsname{0.53}
\expandafter\def\csname diagA@reacher@21\endcsname{0.53}
\expandafter\def\csname diagA@reacher@22\endcsname{0.52}
\expandafter\def\csname diagA@reacher@23\endcsname{0.51}
\expandafter\def\csname diagA@reacher@24\endcsname{0.53}
\expandafter\def\csname diagA@reacher@25\endcsname{0.55}
\expandafter\def\csname diagA@reacher@26\endcsname{0.54}
\expandafter\def\csname diagA@reacher@27\endcsname{0.55}
\expandafter\def\csname diagA@reacher@28\endcsname{0.48}
\expandafter\def\csname hops@reacher@25\endcsname{5}
\expandafter\def\csname hops@reacher@50\endcsname{8}
\expandafter\def\csname hops@reacher@75\endcsname{8}
\expandafter\def\csname hops@reacher@100\endcsname{8}
\expandafter\def\csname hops@reacher@150\endcsname{10}
\expandafter\def\csname cubeNT@50\endcsname{56}
\expandafter\def\csname cubeNT@100\endcsname{19}
\expandafter\def\csname cubeNT@150\endcsname{17}
\newcommand{\cubeNever}{37 of 83}
\newcommand{\cubeClose}{12--27\,cm}
\makeatother


==> tables/numbers_contemp.tex <==
% generated by figs/scripts/viz_table_contemp.py; do not edit
\makeatletter
\providecommand{\Cc}[1]{\csname Cc@#1\endcsname}
\providecommand{\Cn}[1]{\csname Cn@#1\endcsname}
\expandafter\def\csname Cc@ap-cube-25\endcsname{84}
\expandafter\def\csname Cn@ap-cube-25\endcsname{1}
\expandafter\def\csname Cc@ap-cube-50\endcsname{70}
\expandafter\def\csname Cn@ap-cube-50\endcsname{1}
\expandafter\def\csname Cc@ap-cube-100\endcsname{60}
\expandafter\def\csname Cn@ap-cube-100\endcsname{1}
\expandafter\def\csname Cc@ap-cube-150\endcsname{56}
\expandafter\def\csname Cn@ap-cube-150\endcsname{1}
\expandafter\def\csname Cc@ap-pml-50\endcsname{17}
\expandafter\def\csname Cn@ap-pml-50\endcsname{2}
\expandafter\def\csname Cc@ap-pml-100\endcsname{11}
\expandafter\def\csname Cn@ap-pml-100\endcsname{2}
\expandafter\def\csname Cc@ap-pml-200\endcsname{16}
\expandafter\def\csname Cn@ap-pml-200\endcsname{4}
\expandafter\def\csname Cc@ap-pml-400\endcsname{12}
\expandafter\def\csname Cn@ap-pml-400\endcsname{4}
\expandafter\def\csname Cc@ap-pmm-50\endcsname{96}
\expandafter\def\csname Cn@ap-pmm-50\endcsname{3}
\expandafter\def\csname Cc@ap-pmm-100\endcsname{91}
\expandafter\def\csname Cn@ap-pmm-100\endcsname{8}
\expandafter\def\csname Cc@ap-pmm-150\endcsname{88}
\expandafter\def\csname Cn@ap-pmm-150\endcsname{3}
\expandafter\def\csname Cc@ap-pmm-200\endcsname{80}
\expandafter\def\csname Cn@ap-pmm-200\endcsname{8}
\expandafter\def\csname Cc@ap-pusht-50\endcsname{82}
\expandafter\def\csname Cn@ap-pusht-50\endcsname{1}
\expandafter\def\csname Cc@ap-pusht-75\endcsname{66}
\expandafter\def\csname Cn@ap-pusht-75\endcsname{1}
\expandafter\def\csname Cc@ap-pusht-100\endcsname{86}
\expandafter\def\csname Cn@ap-pusht-100\endcsname{1}
\expandafter\def\csname Cc@ap-pusht-150\endcsname{66}
\expandafter\def\csname Cn@ap-pusht-150\endcsname{1}
\expandafter\def\csname Cc@ap-reacher-25\endcsname{44}
\expandafter\def\csname Cn@ap-reacher-25\endcsname{1}
\expandafter\def\csname Cc@ap-reacher-50\endcsname{38}
\expandafter\def\csname Cn@ap-reacher-50\endcsname{1}
\expandafter\def\csname Cc@ap-reacher-100\endcsname{42}
\expandafter\def\csname Cn@ap-reacher-100\endcsname{1}
\expandafter\def\csname Cc@ap-reacher-150\endcsname{34}
\expandafter\def\csname Cn@ap-reacher-150\endcsname{1}
\expandafter\def\csname Cc@ap-tworoom-25\endcsname{98}
\expandafter\def\csname Cn@ap-tworoom-25\endcsname{3}
\expandafter\def\csname Cc@ap-tworoom-50\endcsname{94}
\expandafter\def\csname Cn@ap-tworoom-50\endcsname{6}
\expandafter\def\csname Cc@ap-tworoom-75\endcsname{97}
\expandafter\def\csname Cn@ap-tworoom-75\endcsname{7}
\expandafter\def\csname Cc@apx0p25-pmm-100\endcsname{47}
\expandafter\def\csname Cn@apx0p25-pmm-100\endcsname{2}
\expandafter\def\csname Cc@apx0p25-pmm-200\endcsname{29}
\expandafter\def\csname Cn@apx0p25-pmm-200\endcsname{2}
\expandafter\def\csname Cc@apx0p25-tworoom-75\endcsname{36}
\expandafter\def\csname Cn@apx0p25-tworoom-75\endcsname{1}
\expandafter\def\csname Cc@apx0p5-pml-200\endcsname{17}
\expandafter\def\csname Cn@apx0p5-pml-200\endcsname{2}
\expandafter\def\csname Cc@apx0p5-pml-400\endcsname{11}
\expandafter\def\csname Cn@apx0p5-pml-400\endcsname{2}
\expandafter\def\csname Cc@apx0p5-pmm-100\endcsname{59}
\expandafter\def\csname Cn@apx0p5-pmm-100\endcsname{6}
\expandafter\def\csname Cc@apx0p5-pmm-200\endcsname{29}
\expandafter\def\csname Cn@apx0p5-pmm-200\endcsname{6}
\expandafter\def\csname Cc@apx0p5-tworoom-50\endcsname{86}
\expandafter\def\csname Cn@apx0p5-tworoom-50\endcsname{4}
\expandafter\def\csname Cc@apx0p5-tworoom-75\endcsname{82}
\expandafter\def\csname Cn@apx0p5-tworoom-75\endcsname{5}
\expandafter\def\csname Cc@apx0p75-pmm-100\endcsname{95}
\expandafter\def\csname Cn@apx0p75-pmm-100\endcsname{2}
\expandafter\def\csname Cc@apx0p75-pmm-200\endcsname{54}
\expandafter\def\csname Cn@apx0p75-pmm-200\endcsname{2}
\expandafter\def\csname Cc@apx0p75-tworoom-75\endcsname{98}
\expandafter\def\csname Cn@apx0p75-tworoom-75\endcsname{1}
\expandafter\def\csname Cc@apx1p5-pmm-100\endcsname{74}
\expandafter\def\csname Cn@apx1p5-pmm-100\endcsname{2}
\expandafter\def\csname Cc@apx1p5-pmm-200\endcsname{70}
\expandafter\def\csname Cn@apx1p5-pmm-200\endcsname{2}
\expandafter\def\csname Cc@apx1p5-tworoom-75\endcsname{98}
\expandafter\def\csname Cn@apx1p5-tworoom-75\endcsname{1}
\expandafter\def\csname Cc@apx2-pml-200\endcsname{17}
\expandafter\def\csname Cn@apx2-pml-200\endcsname{2}
\expandafter\def\csname Cc@apx2-pml-400\endcsname{14}
\expandafter\def\csname Cn@apx2-pml-400\endcsname{2}
\expandafter\def\csname Cc@apx2-pmm-100\endcsname{53}
\expandafter\def\csname Cn@apx2-pmm-100\endcsname{6}
\expandafter\def\csname Cc@apx2-pmm-200\endcsname{45}
\expandafter\def\csname Cn@apx2-pmm-200\endcsname{6}
\expandafter\def\csname Cc@apx2-tworoom-50\endcsname{98}
\expandafter\def\csname Cn@apx2-tworoom-50\endcsname{4}
\expandafter\def\csname Cc@apx2-tworoom-75\endcsname{96}
\expandafter\def\csname Cn@apx2-tworoom-75\endcsname{4}
\expandafter\def\csname Cc@apx3-pmm-100\endcsname{15}
\expandafter\def\csname Cn@apx3-pmm-100\endcsname{2}
\expandafter\def\csname Cc@apx3-pmm-200\endcsname{11}
\expandafter\def\csname Cn@apx3-pmm-200\endcsname{2}
\expandafter\def\csname Cc@apx3-tworoom-75\endcsname{2}
\expandafter\def\csname Cn@apx3-tworoom-75\endcsname{1}
\expandafter\def\csname Cc@match1-pmm-200\endcsname{48}
\expandafter\def\csname Cn@match1-pmm-200\endcsname{1}
\expandafter\def\csname Cc@match1-tworoom-75\endcsname{4}
\expandafter\def\csname Cn@match1-tworoom-75\endcsname{1}
\expandafter\def\csname Cc@match2-pmm-200\endcsname{92}
\expandafter\def\csname Cn@match2-pmm-200\endcsname{1}
\expandafter\def\csname Cc@match2-tworoom-75\endcsname{76}
\expandafter\def\csname Cn@match2-tworoom-75\endcsname{1}
\expandafter\def\csname Cc@match3-pmm-200\endcsname{92}
\expandafter\def\csname Cn@match3-pmm-200\endcsname{1}
\expandafter\def\csname Cc@match3-tworoom-75\endcsname{82}
\expandafter\def\csname Cn@match3-tworoom-75\endcsname{1}
\expandafter\def\csname Cc@match4-pmm-200\endcsname{88}
\expandafter\def\csname Cn@match4-pmm-200\endcsname{1}
\expandafter\def\csname Cc@match4-tworoom-75\endcsname{96}
\expandafter\def\csname Cn@match4-tworoom-75\endcsname{1}
\expandafter\def\csname Cc@match6-pmm-200\endcsname{86}
\expandafter\def\csname Cn@match6-pmm-200\endcsname{1}
\expandafter\def\csname Cc@match6-tworoom-75\endcsname{86}
\expandafter\def\csname Cn@match6-tworoom-75\endcsname{1}
\expandafter\def\csname Cc@metro-pmm-50\endcsname{98}
\expandafter\def\csname Cn@metro-pmm-50\endcsname{3}
\expandafter\def\csname Cc@metro-pmm-100\endcsname{95}
\expandafter\def\csname Cn@metro-pmm-100\endcsname{3}
\expandafter\def\csname Cc@metro-pmm-150\endcsname{97}
\expandafter\def\csname Cn@metro-pmm-150\endcsname{3}
\expandafter\def\csname Cc@metro-pmm-200\endcsname{96}
\expandafter\def\csname Cn@metro-pmm-200\endcsname{3}
\expandafter\def\csname Cc@metro-pusht-50\endcsname{72}
\expandafter\def\csname Cn@metro-pusht-50\endcsname{3}
\expandafter\def\csname Cc@metro-pusht-75\endcsname{54}
\expandafter\def\csname Cn@metro-pusht-75\endcsname{3}
\expandafter\def\csname Cc@metro-pusht-150\endcsname{33}
\expandafter\def\csname Cn@metro-pusht-150\endcsname{3}
\expandafter\def\csname Cc@metro-tworoom-25\endcsname{99}
\expandafter\def\csname Cn@metro-tworoom-25\endcsname{3}
\expandafter\def\csname Cc@metro-tworoom-50\endcsname{99}
\expandafter\def\csname Cn@metro-tworoom-50\endcsname{3}
\expandafter\def\csname Cc@metro-tworoom-75\endcsname{99}
\expandafter\def\csname Cn@metro-tworoom-75\endcsname{3}
\expandafter\def\csname Cc@metroours30-pmm-200\endcsname{90}
\expandafter\def\csname Cn@metroours30-pmm-200\endcsname{2}
\expandafter\def\csname Cc@metroours30-pusht-75\endcsname{44}
\expandafter\def\csname Cn@metroours30-pusht-75\endcsname{2}
\expandafter\def\csname Cc@metroours30-tworoom-75\endcsname{77}
\expandafter\def\csname Cn@metroours30-tworoom-75\endcsname{2}
\expandafter\def\csname Cc@metropt10-pmm-200\endcsname{64}
\expandafter\def\csname Cn@metropt10-pmm-200\endcsname{1}
\expandafter\def\csname Cc@metropt10-tworoom-75\endcsname{100}
\expandafter\def\csname Cn@metropt10-tworoom-75\endcsname{1}
\expandafter\def\csname Cc@metropt20-pmm-200\endcsname{76}
\expandafter\def\csname Cn@metropt20-pmm-200\endcsname{1}
\expandafter\def\csname Cc@metropt20-tworoom-75\endcsname{98}
\expandafter\def\csname Cn@metropt20-tworoom-75\endcsname{1}
\expandafter\def\csname Cc@metropt30-pmm-200\endcsname{86}
\expandafter\def\csname Cn@metropt30-pmm-200\endcsname{1}
\expandafter\def\csname Cc@metropt30-tworoom-75\endcsname{70}
\expandafter\def\csname Cn@metropt30-tworoom-75\endcsname{1}
\expandafter\def\csname Cc@mp1-pmm-200\endcsname{48}
\expandafter\def\csname Cn@mp1-pmm-200\endcsname{1}
\expandafter\def\csname Cc@mp1-tworoom-75\endcsname{4}
\expandafter\def\csname Cn@mp1-tworoom-75\endcsname{1}
\expandafter\def\csname Cc@mp2-pmm-200\endcsname{92}
\expandafter\def\csname Cn@mp2-pmm-200\endcsname{1}
\expandafter\def\csname Cc@mp2-tworoom-75\endcsname{92}
\expandafter\def\csname Cn@mp2-tworoom-75\endcsname{1}
\expandafter\def\csname Cc@mp3-pmm-200\endcsname{92}
\expandafter\def\csname Cn@mp3-pmm-200\endcsname{1}
\expandafter\def\csname Cc@mp3-tworoom-75\endcsname{100}
\expandafter\def\csname Cn@mp3-tworoom-75\endcsname{1}
\expandafter\def\csname Cc@mp4-pmm-200\endcsname{88}
\expandafter\def\csname Cn@mp4-pmm-200\endcsname{1}
\expandafter\def\csname Cc@mp4-tworoom-75\endcsname{100}
\expandafter\def\csname Cn@mp4-tworoom-75\endcsname{1}
\expandafter\def\csname Cc@mp6-pmm-200\endcsname{94}
\expandafter\def\csname Cn@mp6-pmm-200\endcsname{1}
\expandafter\def\csname Cc@mp6-tworoom-75\endcsname{94}
\expandafter\def\csname Cn@mp6-tworoom-75\endcsname{1}
\expandafter\def\csname Cc@ngc-cube-25\endcsname{85}
\expandafter\def\csname Cn@ngc-cube-25\endcsname{2}
\expandafter\def\csname Cc@ngc-cube-50\endcsname{69}
\expandafter\def\csname Cn@ngc-cube-50\endcsname{2}
\expandafter\def\csname Cc@ngc-cube-100\endcsname{74}
\expandafter\def\csname Cn@ngc-cube-100\endcsname{2}
\expandafter\def\csname Cc@ngc-cube-150\endcsname{58}
\expandafter\def\csname Cn@ngc-cube-150\endcsname{2}
\expandafter\def\csname Cc@ngc-pmm-50\endcsname{94}
\expandafter\def\csname Cn@ngc-pmm-50\endcsname{2}
\expandafter\def\csname Cc@ngc-pmm-100\endcsname{97}
\expandafter\def\csname Cn@ngc-pmm-100\endcsname{2}
\expandafter\def\csname Cc@ngc-pmm-150\endcsname{95}
\expandafter\def\csname Cn@ngc-pmm-150\endcsname{2}
\expandafter\def\csname Cc@ngc-pmm-200\endcsname{100}
\expandafter\def\csname Cn@ngc-pmm-200\endcsname{2}
\expandafter\def\csname Cc@ngc-pusht-50\endcsname{59}
\expandafter\def\csname Cn@ngc-pusht-50\endcsname{2}
\expandafter\def\csname Cc@ngc-pusht-100\endcsname{23}
\expandafter\def\csname Cn@ngc-pusht-100\endcsname{2}
\expandafter\def\csname Cc@ngc-pusht-150\endcsname{11}
\expandafter\def\csname Cn@ngc-pusht-150\endcsname{2}
\expandafter\def\csname Cc@ngc-reacher-25\endcsname{66}
\expandafter\def\csname Cn@ngc-reacher-25\endcsname{2}
\expandafter\def\csname Cc@ngc-reacher-50\endcsname{71}
\expandafter\def\csname Cn@ngc-reacher-50\endcsname{2}
\expandafter\def\csname Cc@ngc-reacher-100\endcsname{85}
\expandafter\def\csname Cn@ngc-reacher-100\endcsname{2}
\expandafter\def\csname Cc@ngc-reacher-150\endcsname{75}
\expandafter\def\csname Cn@ngc-reacher-150\endcsname{2}
\expandafter\def\csname Cc@ngc-tworoom-25\endcsname{100}
\expandafter\def\csname Cn@ngc-tworoom-25\endcsname{2}
\expandafter\def\csname Cc@ngc-tworoom-50\endcsname{100}
\expandafter\def\csname Cn@ngc-tworoom-50\endcsname{2}
\expandafter\def\csname Cc@ngc-tworoom-75\endcsname{99}
\expandafter\def\csname Cn@ngc-tworoom-75\endcsname{2}
\expandafter\def\csname Cc@pass1-pmm-200\endcsname{22}
\expandafter\def\csname Cn@pass1-pmm-200\endcsname{1}
\expandafter\def\csname Cc@pass1-tworoom-75\endcsname{10}
\expandafter\def\csname Cn@pass1-tworoom-75\endcsname{1}
\expandafter\def\csname Cc@pass2-pmm-200\endcsname{60}
\expandafter\def\csname Cn@pass2-pmm-200\endcsname{1}
\expandafter\def\csname Cc@pass2-tworoom-75\endcsname{92}
\expandafter\def\csname Cn@pass2-tworoom-75\endcsname{1}
\expandafter\def\csname Cc@pass3-pmm-200\endcsname{72}
\expandafter\def\csname Cn@pass3-pmm-200\endcsname{1}
\expandafter\def\csname Cc@pass3-tworoom-75\endcsname{100}
\expandafter\def\csname Cn@pass3-tworoom-75\endcsname{1}
\expandafter\def\csname Cc@pass4-pmm-200\endcsname{82}
\expandafter\def\csname Cn@pass4-pmm-200\endcsname{1}
\expandafter\def\csname Cc@pass4-tworoom-75\endcsname{100}
\expandafter\def\csname Cn@pass4-tworoom-75\endcsname{1}
\expandafter\def\csname Cc@pass6-pmm-200\endcsname{80}
\expandafter\def\csname Cn@pass6-pmm-200\endcsname{1}
\expandafter\def\csname Cc@pass6-tworoom-75\endcsname{92}
\expandafter\def\csname Cn@pass6-tworoom-75\endcsname{1}
\expandafter\def\csname Cc@sweep-pmm-100-3x20\endcsname{96}
\expandafter\def\csname Cc@sweep-pmm-150-3x20\endcsname{98}
\expandafter\def\csname Cc@sweep-pmm-200-1x10\endcsname{96}
\expandafter\def\csname Cc@sweep-pmm-200-1x5\endcsname{82}
\expandafter\def\csname Cc@sweep-pmm-200-3x15\endcsname{92}
\expandafter\def\csname Cc@sweep-pmm-200-3x20\endcsname{98}
\expandafter\def\csname Cc@sweep-pmm-200-5x25\endcsname{96}
\expandafter\def\csname Cc@sweep-pmm-200-5x30\endcsname{90}
\expandafter\def\csname Cc@sweep-pmm-50-3x20\endcsname{96}
\expandafter\def\csname Cc@sweep-pusht-150-3x20\endcsname{24}
\expandafter\def\csname Cc@sweep-pusht-50-3x20\endcsname{68}
\expandafter\def\csname Cc@sweep-pusht-75-1x10\endcsname{36}
\expandafter\def\csname Cc@sweep-pusht-75-1x5\endcsname{24}
\expandafter\def\csname Cc@sweep-pusht-75-3x15\endcsname{50}
\expandafter\def\csname Cc@sweep-pusht-75-3x20\endcsname{58}
\expandafter\def\csname Cc@sweep-pusht-75-5x25\endcsname{58}
\expandafter\def\csname Cc@sweep-pusht-75-5x30\endcsname{56}
\expandafter\def\csname Cc@sweep-tworoom-25-1x10\endcsname{100}
\expandafter\def\csname Cc@sweep-tworoom-50-1x10\endcsname{100}
\expandafter\def\csname Cc@sweep-tworoom-75-1x10\endcsname{100}
\expandafter\def\csname Cc@sweep-tworoom-75-1x5\endcsname{22}
\expandafter\def\csname Cc@sweep-tworoom-75-3x15\endcsname{96}
\expandafter\def\csname Cc@sweep-tworoom-75-3x20\endcsname{72}
\expandafter\def\csname Cc@sweep-tworoom-75-5x25\endcsname{42}
\expandafter\def\csname Cc@sweep-tworoom-75-5x30\endcsname{30}
\makeatother


==> tables/numbers_e1.tex <==
% generated by figs/scripts/fig_e1_range.py; do not edit
\makeatletter
\providecommand{\Ea}[1]{\csname Ea@#1\endcsname}
\expandafter\def\csname Ea@pmm-pixels-1\endcsname{0.96}
\expandafter\def\csname Ea@pmm-pixels-3\endcsname{0.69}
\expandafter\def\csname Ea@pmm-pixels-6\endcsname{0.56}
\expandafter\def\csname Ea@pmm-lewm-1\endcsname{0.98}
\expandafter\def\csname Ea@pmm-lewm-3\endcsname{0.73}
\expandafter\def\csname Ea@pmm-lewm-6\endcsname{0.65}
\expandafter\def\csname Ea@pmm-dinov2-1\endcsname{0.94}
\expandafter\def\csname Ea@pmm-dinov2-3\endcsname{0.67}
\expandafter\def\csname Ea@pmm-dinov2-6\endcsname{0.54}
\expandafter\def\csname Ea@pmm-clip-1\endcsname{0.94}
\expandafter\def\csname Ea@pmm-clip-3\endcsname{0.67}
\expandafter\def\csname Ea@pmm-clip-6\endcsname{0.56}
\expandafter\def\csname Ea@pmm-siglip-1\endcsname{0.96}
\expandafter\def\csname Ea@pmm-siglip-3\endcsname{0.69}
\expandafter\def\csname Ea@pmm-siglip-6\endcsname{0.59}
\expandafter\def\csname Ea@pmm-vjepa2-1\endcsname{0.85}
\expandafter\def\csname Ea@pmm-vjepa2-3\endcsname{0.59}
\expandafter\def\csname Ea@pmm-vjepa2-6\endcsname{0.52}
\expandafter\def\csname Ea@pmm-pldm-1\endcsname{0.98}
\expandafter\def\csname Ea@pmm-pldm-3\endcsname{0.71}
\expandafter\def\csname Ea@pmm-pldm-6\endcsname{0.56}
\expandafter\def\csname Ea@pmm-pldm-12\endcsname{0.52}
\expandafter\def\csname Ea@pmm-pldm5-1\endcsname{0.97}
\expandafter\def\csname Ea@pmm-pldm5-3\endcsname{0.72}
\expandafter\def\csname Ea@pmm-pldm5-6\endcsname{0.54}
\expandafter\def\csname Ea@pmm-pldm5-12\endcsname{0.52}
\expandafter\def\csname Ea@tworoom-pixels-1\endcsname{0.99}
\expandafter\def\csname Ea@tworoom-pixels-3\endcsname{0.67}
\expandafter\def\csname Ea@tworoom-pixels-6\endcsname{0.56}
\expandafter\def\csname Ea@tworoom-lewm-1\endcsname{0.97}
\expandafter\def\csname Ea@tworoom-lewm-3\endcsname{0.63}
\expandafter\def\csname Ea@tworoom-lewm-6\endcsname{0.50}
\expandafter\def\csname Ea@tworoom-dinov2-1\endcsname{0.93}
\expandafter\def\csname Ea@tworoom-dinov2-3\endcsname{0.63}
\expandafter\def\csname Ea@tworoom-dinov2-6\endcsname{0.55}
\expandafter\def\csname Ea@tworoom-clip-1\endcsname{0.93}
\expandafter\def\csname Ea@tworoom-clip-3\endcsname{0.63}
\expandafter\def\csname Ea@tworoom-clip-6\endcsname{0.56}
\expandafter\def\csname Ea@tworoom-siglip-1\endcsname{0.96}
\expandafter\def\csname Ea@tworoom-siglip-3\endcsname{0.64}
\expandafter\def\csname Ea@tworoom-siglip-6\endcsname{0.57}
\expandafter\def\csname Ea@tworoom-vjepa2-1\endcsname{0.88}
\expandafter\def\csname Ea@tworoom-vjepa2-3\endcsname{0.60}
\expandafter\def\csname Ea@tworoom-vjepa2-6\endcsname{0.56}
\expandafter\def\csname Ea@pmm-r6lo\endcsname{0.52}
\expandafter\def\csname Ea@pmm-r6hi\endcsname{0.65}
\expandafter\def\csname Ea@pmm-r1lo\endcsname{0.85}
\expandafter\def\csname Ea@pmm-r1hi\endcsname{0.98}
\expandafter\def\csname Ea@pmm-hlo\endcsname{5}
\expandafter\def\csname Ea@pmm-hhi\endcsname{10}
\expandafter\def\csname Ea@tworoom-r6lo\endcsname{0.50}
\expandafter\def\csname Ea@tworoom-r6hi\endcsname{0.57}
\expandafter\def\csname Ea@tworoom-r1lo\endcsname{0.88}
\expandafter\def\csname Ea@tworoom-r1hi\endcsname{0.99}
\expandafter\def\csname Ea@tworoom-hlo\endcsname{5}
\expandafter\def\csname Ea@tworoom-hhi\endcsname{10}
\expandafter\def\csname Ea@pmm-lewm-12\endcsname{0.44}
\makeatother


==> tables/numbers_e2.tex <==
% generated by figs/scripts/fig_e2_epochs.py; do not edit
\makeatletter
\providecommand{\Ec}[1]{\csname Ec@#1\endcsname}
\expandafter\def\csname Ec@ep1-1\endcsname{0.98}
\expandafter\def\csname Ec@ep10-1\endcsname{0.99}
\expandafter\def\csname Ec@max-1\endcsname{0.99}
\expandafter\def\csname Ec@min-1\endcsname{0.98}
\expandafter\def\csname Ec@pix-1\endcsname{0.97}
\expandafter\def\csname Ec@ep1-3\endcsname{0.66}
\expandafter\def\csname Ec@ep10-3\endcsname{0.68}
\expandafter\def\csname Ec@max-3\endcsname{0.68}
\expandafter\def\csname Ec@min-3\endcsname{0.66}
\expandafter\def\csname Ec@pix-3\endcsname{0.68}
\expandafter\def\csname Ec@ep1-6\endcsname{0.55}
\expandafter\def\csname Ec@ep10-6\endcsname{0.57}
\expandafter\def\csname Ec@max-6\endcsname{0.57}
\expandafter\def\csname Ec@min-6\endcsname{0.55}
\expandafter\def\csname Ec@pix-6\endcsname{0.59}
\expandafter\def\csname Ec@ep1-12\endcsname{0.51}
\expandafter\def\csname Ec@ep10-12\endcsname{0.49}
\expandafter\def\csname Ec@max-12\endcsname{0.51}
\expandafter\def\csname Ec@min-12\endcsname{0.49}
\expandafter\def\csname Ec@pix-12\endcsname{0.53}
\expandafter\def\csname Ec@hlo\endcsname{6}
\expandafter\def\csname Ec@hhi\endcsname{8}
\expandafter\def\csname Ec@neps\endcsname{10}
\makeatother


==> tables/numbers_e3b.tex <==
% generated by figs/scripts/figS8_exchange.py; do not edit
\makeatletter
\providecommand{\Eb}[1]{\csname Eb@#1\endcsname}
\expandafter\def\csname Eb@pixel-lo\endcsname{6.3}
\expandafter\def\csname Eb@pixel-hi\endcsname{35}
\expandafter\def\csname Eb@pixel-above\endcsname{9}
\expandafter\def\csname Eb@dinov2-lo\endcsname{2.6}
\expandafter\def\csname Eb@dinov2-hi\endcsname{14}
\expandafter\def\csname Eb@dinov2-above\endcsname{9}
\expandafter\def\csname Eb@clip-lo\endcsname{1.0}
\expandafter\def\csname Eb@clip-hi\endcsname{16}
\expandafter\def\csname Eb@clip-above\endcsname{8}
\expandafter\def\csname Eb@siglip-lo\endcsname{2.4}
\expandafter\def\csname Eb@siglip-hi\endcsname{9}
\expandafter\def\csname Eb@siglip-above\endcsname{9}
\expandafter\def\csname Eb@vjepa2-lo\endcsname{2.2}
\expandafter\def\csname Eb@vjepa2-hi\endcsname{12}
\expandafter\def\csname Eb@vjepa2-above\endcsname{9}
\expandafter\def\csname Eb@clip-lo2\endcsname{1.9}
\expandafter\def\csname Eb@ntask\endcsname{9}
\makeatother


==> tables/numbers_exp2x.tex <==
% generated by figs/scripts/exp21_23.py -- do not edit
\makeatletter
\expandafter\def\csname R@x21-pmm-best-h5\endcsname{4}
\expandafter\def\csname R@x21-pmm-best-h10\endcsname{6}
\expandafter\def\csname R@x21-pmm-best-h15\endcsname{6}
\expandafter\def\csname R@x21-pmm-k12-h5\endcsname{11}
\expandafter\def\csname R@x21-pmm-k12-h15\endcsname{65}
\expandafter\def\csname R@x21-pmm-k2-h5\endcsname{66}
\expandafter\def\csname R@x21-pmm-k2-h15\endcsname{45}
\expandafter\def\csname R@x21-tworoom-best-h5\endcsname{4}
\expandafter\def\csname R@x21-tworoom-best-h10\endcsname{6}
\expandafter\def\csname R@x21-tworoom-best-h15\endcsname{6}
\expandafter\def\csname R@x21-tworoom-k12-h5\endcsname{39}
\expandafter\def\csname R@x21-tworoom-k12-h15\endcsname{66}
\expandafter\def\csname R@x21-tworoom-k2-h5\endcsname{24}
\expandafter\def\csname R@x21-tworoom-k2-h15\endcsname{11}
\expandafter\def\csname R@x21-gap6\endcsname{6}
\expandafter\def\csname R@x22-pmm-best\endcsname{28}
\expandafter\def\csname R@x22-pmm-besth\endcsname{20}
\expandafter\def\csname R@x22-pmm-bestn\endcsname{1000}
\expandafter\def\csname R@x22-pmm-ours\endcsname{89}
\expandafter\def\csname R@x22-tworoom-best\endcsname{77}
\expandafter\def\csname R@x22-tworoom-besth\endcsname{20}
\expandafter\def\csname R@x22-tworoom-bestn\endcsname{1000}
\expandafter\def\csname R@x22-tworoom-ours\endcsname{94}
\expandafter\def\csname R@x23-pmm-max\endcsname{84}
\expandafter\def\csname R@x23-pmm-far-max\endcsname{21}
\expandafter\def\csname R@x23-pmm-gcbch-far\endcsname{21}
\expandafter\def\csname R@x23-pml-max\endcsname{17}
\expandafter\def\csname R@x23-pml-far-max\endcsname{10}
\expandafter\def\csname R@x23-pml-gcbch-far\endcsname{6}
\makeatother


==> tables/numbers_ext.tex <==
% generated by figs/scripts/make_tables_ext.py -- do not edit
\makeatletter
\newcommand{\R}[1]{\@ifundefined{R@#1}{\textbf{??#1}}{\csname R@#1\endcsname}}
\expandafter\def\csname R@abl-f10\endcsname{79}
\expandafter\def\csname R@abl-f25\endcsname{83}
\expandafter\def\csname R@abl-f50\endcsname{84}
\expandafter\def\csname R@abl-full\endcsname{86}
\expandafter\def\csname R@abl-k20\endcsname{80}
\expandafter\def\csname R@abl-k5\endcsname{80}
\expandafter\def\csname R@abl-knn0\endcsname{6}
\expandafter\def\csname R@abl-knn0-x\endcsname{40}
\expandafter\def\csname R@abl-ours-tworoom\endcsname{96}
\expandafter\def\csname R@abl-q25\endcsname{74}
\expandafter\def\csname R@abl-q75\endcsname{86}
\expandafter\def\csname R@apoff-pmm-100-0.5\endcsname{56}
\expandafter\def\csname R@apoff-pmm-100-1\endcsname{88}
\expandafter\def\csname R@apoff-pmm-100-2\endcsname{62}
\expandafter\def\csname R@apoff-pmm-100-ours\endcsname{84}
\expandafter\def\csname R@apoff-pmm-200-0.5\endcsname{34}
\expandafter\def\csname R@apoff-pmm-200-1\endcsname{80}
\expandafter\def\csname R@apoff-pmm-200-2\endcsname{54}
\expandafter\def\csname R@apoff-pmm-200-ours\endcsname{92}
\expandafter\def\csname R@apoff-tworoom-50-0.5\endcsname{86}
\expandafter\def\csname R@apoff-tworoom-50-1\endcsname{94}
\expandafter\def\csname R@apoff-tworoom-50-2\endcsname{100}
\expandafter\def\csname R@apoff-tworoom-50-ours\endcsname{92}
\expandafter\def\csname R@apoff-tworoom-75-0.5\endcsname{82}
\expandafter\def\csname R@apoff-tworoom-75-1\endcsname{98}
\expandafter\def\csname R@apoff-tworoom-75-2\endcsname{94}
\expandafter\def\csname R@apoff-tworoom-75-ours\endcsname{94}
\expandafter\def\csname R@apoffloss\endcsname{46}
\expandafter\def\csname R@cem-pmm-released\endcsname{12}
\expandafter\def\csname R@cem-pmm-relmin\endcsname{10}
\expandafter\def\csname R@cem-tworoom-released\endcsname{28}
\expandafter\def\csname R@cem-tworoom-relmin\endcsname{54}
\expandafter\def\csname R@cem3x-pmm-released\endcsname{12}
\expandafter\def\csname R@cem3x-pmm-relmin\endcsname{10}
\expandafter\def\csname R@cem3x-tworoom-released\endcsname{36}
\expandafter\def\csname R@cem3x-tworoom-relmin\endcsname{56}
\expandafter\def\csname R@cube-ho-100\endcsname{57}
\expandafter\def\csname R@cube-ho-150\endcsname{31}
\expandafter\def\csname R@cube-ho-50\endcsname{58}
\expandafter\def\csname R@cube-ho-ours-100\endcsname{56}
\expandafter\def\csname R@cube-ho-ours-150\endcsname{29}
\expandafter\def\csname R@cube-ho-ours-50\endcsname{57}
\expandafter\def\csname R@cube-ho-released-100\endcsname{56}
\expandafter\def\csname R@cube-ho-released-150\endcsname{19}
\expandafter\def\csname R@cube-ho-released-50\endcsname{57}
\expandafter\def\csname R@cube-ho-relmin-100\endcsname{57}
\expandafter\def\csname R@cube-ho-relmin-150\endcsname{24}
\expandafter\def\csname R@cube-ho-relmin-50\endcsname{53}
\expandafter\def\csname R@dropmax\endcsname{83}
\expandafter\def\csname R@dropmin\endcsname{37}
\expandafter\def\csname R@gain-pmm-200\endcsname{71}
\expandafter\def\csname R@gain-relmin-tworoom-75\endcsname{31}
\expandafter\def\csname R@gain-tworoom-75\endcsname{62}
\expandafter\def\csname R@gap-x\endcsname{21}
\expandafter\def\csname R@ho-reacher-ours-100\endcsname{66}
\expandafter\def\csname R@ho-reacher-ours-150\endcsname{68}
\expandafter\def\csname R@ho-reacher-released-100\endcsname{70}
\expandafter\def\csname R@ho-reacher-released-150\endcsname{60}
\expandafter\def\csname R@ho-reacher-relmin-100\endcsname{73}
\expandafter\def\csname R@ho-reacher-relmin-150\endcsname{77}
\expandafter\def\csname R@ho0-pmm-200\endcsname{88}
\expandafter\def\csname R@ho0-reacher-100\endcsname{88}
\expandafter\def\csname R@ho0-reacher-150\endcsname{82}
\expandafter\def\csname R@ho0-reacher-25\endcsname{82}
\expandafter\def\csname R@ho0-reacher-50\endcsname{80}
\expandafter\def\csname R@ho0-tworoom-75\endcsname{72}
\expandafter\def\csname R@ho12-gain-reacher\endcsname{2}
\expandafter\def\csname R@ho12-gain-reacher-100\endcsname{12}
\expandafter\def\csname R@ho12-gain-reacher-150\endcsname{2}
\expandafter\def\csname R@ho12-gainmax-reacher\endcsname{12}
\expandafter\def\csname R@ho12-pmm-200\endcsname{86}
\expandafter\def\csname R@ho12-pusht-100\endcsname{45}
\expandafter\def\csname R@ho12-pusht-150\endcsname{35}
\expandafter\def\csname R@ho12-reacher-100\endcsname{86}
\expandafter\def\csname R@ho12-reacher-150\endcsname{80}
\expandafter\def\csname R@ho12-reacher-25\endcsname{73}
\expandafter\def\csname R@ho12-reacher-50\endcsname{75}
\expandafter\def\csname R@ho12-tworoom-75\endcsname{87}
\expandafter\def\csname R@ho8-reacher-100\endcsname{70}
\expandafter\def\csname R@ho8-reacher-150\endcsname{64}
\expandafter\def\csname R@ho8-tworoom-75\endcsname{92}
\expandafter\def\csname R@pldm-pmm-ours-100\endcsname{28}
\expandafter\def\csname R@pldm-pmm-ours-200\endcsname{4}
\expandafter\def\csname R@pldm-pmm-ours-x\endcsname{28}
\expandafter\def\csname R@pldm-pmm-released-100\endcsname{17}
\expandafter\def\csname R@pldm-pmm-released-200\endcsname{3}
\expandafter\def\csname R@pldm-pmm-released-x\endcsname{28}
\expandafter\def\csname R@pldm-pmm-relmin-100\endcsname{12}
\expandafter\def\csname R@pldm-pmm-relmin-200\endcsname{4}
\expandafter\def\csname R@pldm-tworoom-ours-25\endcsname{95}
\expandafter\def\csname R@pldm-tworoom-ours-50\endcsname{98}
\expandafter\def\csname R@pldm-tworoom-ours-75\endcsname{97}
\expandafter\def\csname R@pldm-tworoom-ours-x\endcsname{99}
\expandafter\def\csname R@pldm-tworoom-released-25\endcsname{98}
\expandafter\def\csname R@pldm-tworoom-released-50\endcsname{75}
\expandafter\def\csname R@pldm-tworoom-released-75\endcsname{50}
\expandafter\def\csname R@pldm-tworoom-released-x\endcsname{81}
\expandafter\def\csname R@pldm-tworoom-relmin-25\endcsname{100}
\expandafter\def\csname R@pldm-tworoom-relmin-50\endcsname{85}
\expandafter\def\csname R@pldm-tworoom-relmin-75\endcsname{62}
\expandafter\def\csname R@pml-ap-100\endcsname{11}
\expandafter\def\csname R@pml-ap-200\endcsname{16}
\expandafter\def\csname R@pml-ap-400\endcsname{12}
\expandafter\def\csname R@pml-ap-50\endcsname{17}
\expandafter\def\csname R@pml-ap-x\endcsname{6}
\expandafter\def\csname R@pml-dwm-200\endcsname{95}
\expandafter\def\csname R@pml-dwm-400\endcsname{100}
\expandafter\def\csname R@pml-dwm-x\endcsname{100}
\expandafter\def\csname R@pml-gcbc-100\endcsname{25}
\expandafter\def\csname R@pml-gcbc-200\endcsname{18}
\expandafter\def\csname R@pml-gcbc-400\endcsname{18}
\expandafter\def\csname R@pml-gcbc-50\endcsname{33}
\expandafter\def\csname R@pml-gcbc-x\endcsname{17}
\expandafter\def\csname R@pml-gciql-100\endcsname{8}
\expandafter\def\csname R@pml-gciql-200\endcsname{9}
\expandafter\def\csname R@pml-gciql-400\endcsname{3}
\expandafter\def\csname R@pml-gciql-50\endcsname{9}
\expandafter\def\csname R@pml-gciql-x\endcsname{3}
\expandafter\def\csname R@pml-gcivl-100\endcsname{8}
\expandafter\def\csname R@pml-gcivl-200\endcsname{9}
\expandafter\def\csname R@pml-gcivl-400\endcsname{1}
\expandafter\def\csname R@pml-gcivl-50\endcsname{9}
\expandafter\def\csname R@pml-gcivl-x\endcsname{3}
\expandafter\def\csname R@pml-hilp-100\endcsname{13}
\expandafter\def\csname R@pml-hilp-200\endcsname{16}
\expandafter\def\csname R@pml-hilp-400\endcsname{9}
\expandafter\def\csname R@pml-hilp-50\endcsname{12}
\expandafter\def\csname R@pml-hilp-x\endcsname{10}
\expandafter\def\csname R@pml-ours-100\endcsname{63}
\expandafter\def\csname R@pml-ours-200\endcsname{73}
\expandafter\def\csname R@pml-ours-400\endcsname{87}
\expandafter\def\csname R@pml-ours-50\endcsname{62}
\expandafter\def\csname R@pml-ours-x\endcsname{66}
\expandafter\def\csname R@pml-pldm-100\endcsname{10}
\expandafter\def\csname R@pml-pldm-200\endcsname{10}
\expandafter\def\csname R@pml-pldm-400\endcsname{1}
\expandafter\def\csname R@pml-pldm-50\endcsname{9}
\expandafter\def\csname R@pml-pldm-x\endcsname{2}
\expandafter\def\csname R@pml-released-100\endcsname{15}
\expandafter\def\csname R@pml-released-200\endcsname{13}
\expandafter\def\csname R@pml-released-400\endcsname{8}
\expandafter\def\csname R@pml-released-50\endcsname{14}
\expandafter\def\csname R@pml-released-x\endcsname{5}
\expandafter\def\csname R@pml-relmin-100\endcsname{28}
\expandafter\def\csname R@pml-relmin-200\endcsname{23}
\expandafter\def\csname R@pml-relmin-400\endcsname{26}
\expandafter\def\csname R@pml-relmin-50\endcsname{44}
\expandafter\def\csname R@pml-relmin-x\endcsname{17}
\expandafter\def\csname R@pmm-ap-100\endcsname{92}
\expandafter\def\csname R@pmm-ap-150\endcsname{88}
\expandafter\def\csname R@pmm-ap-200\endcsname{81}
\expandafter\def\csname R@pmm-ap-50\endcsname{96}
\expandafter\def\csname R@pmm-ap-x\endcsname{73}
\expandafter\def\csname R@pmm-dwm-100\endcsname{70}
\expandafter\def\csname R@pmm-dwm-200\endcsname{15}
\expandafter\def\csname R@pmm-dwm-x\endcsname{35}
\expandafter\def\csname R@pmm-gcbc-100\endcsname{83}
\expandafter\def\csname R@pmm-gcbc-150\endcsname{54}
\expandafter\def\csname R@pmm-gcbc-200\endcsname{51}
\expandafter\def\csname R@pmm-gcbc-50\endcsname{93}
\expandafter\def\csname R@pmm-gcbc-x\endcsname{51}
\expandafter\def\csname R@pmm-gciql-100\endcsname{4}
\expandafter\def\csname R@pmm-gciql-150\endcsname{0}
\expandafter\def\csname R@pmm-gciql-200\endcsname{1}
\expandafter\def\csname R@pmm-gciql-50\endcsname{34}
\expandafter\def\csname R@pmm-gciql-x\endcsname{12}
\expandafter\def\csname R@pmm-gcivl-100\endcsname{4}
\expandafter\def\csname R@pmm-gcivl-150\endcsname{2}
\expandafter\def\csname R@pmm-gcivl-200\endcsname{0}
\expandafter\def\csname R@pmm-gcivl-50\endcsname{30}
\expandafter\def\csname R@pmm-gcivl-x\endcsname{16}
\expandafter\def\csname R@pmm-hilp-100\endcsname{3}
\expandafter\def\csname R@pmm-hilp-150\endcsname{1}
\expandafter\def\csname R@pmm-hilp-200\endcsname{1}
\expandafter\def\csname R@pmm-hilp-50\endcsname{32}
\expandafter\def\csname R@pmm-hilp-x\endcsname{18}
\expandafter\def\csname R@pmm-ours-100\endcsname{89}
\expandafter\def\csname R@pmm-ours-150\endcsname{88}
\expandafter\def\csname R@pmm-ours-200\endcsname{85}
\expandafter\def\csname R@pmm-ours-50\endcsname{91}
\expandafter\def\csname R@pmm-ours-x\endcsname{95}
\expandafter\def\csname R@pmm-pldm-100\endcsname{17}
\expandafter\def\csname R@pmm-pldm-200\endcsname{3}
\expandafter\def\csname R@pmm-pldm-x\endcsname{28}
\expandafter\def\csname R@pmm-released-100\endcsname{25}
\expandafter\def\csname R@pmm-released-150\endcsname{13}
\expandafter\def\csname R@pmm-released-200\endcsname{13}
\expandafter\def\csname R@pmm-released-50\endcsname{50}
\expandafter\def\csname R@pmm-released-x\endcsname{39}
\expandafter\def\csname R@pmm-relmin-100\endcsname{33}
\expandafter\def\csname R@pmm-relmin-150\endcsname{17}
\expandafter\def\csname R@pmm-relmin-200\endcsname{12}
\expandafter\def\csname R@pmm-relmin-50\endcsname{70}
\expandafter\def\csname R@pmm-relmin-x\endcsname{41}
\expandafter\def\csname R@pol-maze-max\endcsname{16}
\expandafter\def\csname R@pusht-ap-100\endcsname{86}
\expandafter\def\csname R@pusht-ap-150\endcsname{66}
\expandafter\def\csname R@pusht-ap-50\endcsname{82}
\expandafter\def\csname R@pusht-ap-75\endcsname{66}
\expandafter\def\csname R@pusht-gcbc-100\endcsname{11}
\expandafter\def\csname R@pusht-gcbc-150\endcsname{5}
\expandafter\def\csname R@pusht-gcbc-50\endcsname{16}
\expandafter\def\csname R@pusht-gcbc-75\endcsname{8}
\expandafter\def\csname R@pusht-gciql-100\endcsname{0}
\expandafter\def\csname R@pusht-gciql-150\endcsname{0}
\expandafter\def\csname R@pusht-gciql-50\endcsname{0}
\expandafter\def\csname R@pusht-gciql-75\endcsname{0}
\expandafter\def\csname R@pusht-gcivl-100\endcsname{0}
\expandafter\def\csname R@pusht-gcivl-150\endcsname{0}
\expandafter\def\csname R@pusht-gcivl-50\endcsname{2}
\expandafter\def\csname R@pusht-gcivl-75\endcsname{0}
\expandafter\def\csname R@pusht-hilp-100\endcsname{0}
\expandafter\def\csname R@pusht-hilp-150\endcsname{0}
\expandafter\def\csname R@pusht-hilp-50\endcsname{0}
\expandafter\def\csname R@pusht-hilp-75\endcsname{0}
\expandafter\def\csname R@pusht-ours-100\endcsname{40}
\expandafter\def\csname R@pusht-ours-150\endcsname{30}
\expandafter\def\csname R@pusht-ours-50\endcsname{65}
\expandafter\def\csname R@pusht-ours-75\endcsname{50}
\expandafter\def\csname R@pusht-pldm-100\endcsname{0}
\expandafter\def\csname R@pusht-pldm-150\endcsname{0}
\expandafter\def\csname R@pusht-pldm-50\endcsname{2}
\expandafter\def\csname R@pusht-pldm-75\endcsname{0}
\expandafter\def\csname R@pusht-released-100\endcsname{17}
\expandafter\def\csname R@pusht-released-150\endcsname{5}
\expandafter\def\csname R@pusht-released-25\endcsname{88}
\expandafter\def\csname R@pusht-released-50\endcsname{41}
\expandafter\def\csname R@pusht-released-75\endcsname{21}
\expandafter\def\csname R@pusht-relmin-100\endcsname{17}
\expandafter\def\csname R@pusht-relmin-150\endcsname{9}
\expandafter\def\csname R@pusht-relmin-25\endcsname{94}
\expandafter\def\csname R@pusht-relmin-50\endcsname{55}
\expandafter\def\csname R@pusht-relmin-75\endcsname{33}
\expandafter\def\csname R@rand-ap-exp-100\endcsname{90}
\expandafter\def\csname R@rand-ap-exp-150\endcsname{88}
\expandafter\def\csname R@rand-ap-exp-200\endcsname{81}
\expandafter\def\csname R@rand-ap-exp-50\endcsname{96}
\expandafter\def\csname R@rand-ap-exp-x\endcsname{73}
\expandafter\def\csname R@rand-ap-rand-100\endcsname{95}
\expandafter\def\csname R@rand-ap-rand-150\endcsname{57}
\expandafter\def\csname R@rand-ap-rand-200\endcsname{48}
\expandafter\def\csname R@rand-ap-rand-50\endcsname{99}
\expandafter\def\csname R@rand-ap-rand-x\endcsname{73}
\expandafter\def\csname R@rand-ours-exp-100\endcsname{88}
\expandafter\def\csname R@rand-ours-exp-150\endcsname{91}
\expandafter\def\csname R@rand-ours-exp-200\endcsname{86}
\expandafter\def\csname R@rand-ours-exp-50\endcsname{90}
\expandafter\def\csname R@rand-ours-exp-x\endcsname{94}
\expandafter\def\csname R@rand-ours-rand-100\endcsname{90}
\expandafter\def\csname R@rand-ours-rand-150\endcsname{87}
\expandafter\def\csname R@rand-ours-rand-200\endcsname{90}
\expandafter\def\csname R@rand-ours-rand-50\endcsname{95}
\expandafter\def\csname R@rand-ours-rand-x\endcsname{95}
\expandafter\def\csname R@reacher-pldm-150\endcsname{15}
\expandafter\def\csname R@reacher-pldm-25\endcsname{24}
\expandafter\def\csname R@span-pmm-12\endcsname{35}
\expandafter\def\csname R@span-pmm-2\endcsname{57}
\expandafter\def\csname R@span-pmm-4\endcsname{77}
\expandafter\def\csname R@span-pmm-6\endcsname{83}
\expandafter\def\csname R@span-pmm-8\endcsname{75}
\expandafter\def\csname R@span-tworoom-12\endcsname{58}
\expandafter\def\csname R@span-tworoom-2\endcsname{21}
\expandafter\def\csname R@span-tworoom-4\endcsname{75}
\expandafter\def\csname R@span-tworoom-6\endcsname{94}
\expandafter\def\csname R@span-tworoom-8\endcsname{77}
\expandafter\def\csname R@sw3-pml-400\endcsname{92}
\expandafter\def\csname R@sw3-pml-x\endcsname{66}
\expandafter\def\csname R@sw3-pmm-200\endcsname{77}
\expandafter\def\csname R@sw3-pmm-x\endcsname{84}
\expandafter\def\csname R@sw3-pusht-100\endcsname{56}
\expandafter\def\csname R@sw3-pusht-150\endcsname{48}
\expandafter\def\csname R@sw3-reacher-100\endcsname{78}
\expandafter\def\csname R@sw3-reacher-150\endcsname{73}
\expandafter\def\csname R@sw3-tworoom-75\endcsname{83}
\expandafter\def\csname R@sw3-tworoom-x\endcsname{98}
\expandafter\def\csname R@swnav-pml-200\endcsname{68}
\expandafter\def\csname R@swnav-pml-400\endcsname{92}
\expandafter\def\csname R@swnav-pml-x\endcsname{66}
\expandafter\def\csname R@swnav-pmm-100\endcsname{78}
\expandafter\def\csname R@swnav-pmm-200\endcsname{77}
\expandafter\def\csname R@swnav-pmm-x\endcsname{84}
\expandafter\def\csname R@swnav-tworoom-75\endcsname{83}
\expandafter\def\csname R@swnav-tworoom-x\endcsname{98}
\expandafter\def\csname R@tworoom-ap-25\endcsname{98}
\expandafter\def\csname R@tworoom-ap-50\endcsname{93}
\expandafter\def\csname R@tworoom-ap-75\endcsname{97}
\expandafter\def\csname R@tworoom-ap-x\endcsname{96}
\expandafter\def\csname R@tworoom-dwm-50\endcsname{90}
\expandafter\def\csname R@tworoom-dwm-75\endcsname{70}
\expandafter\def\csname R@tworoom-dwm-x\endcsname{95}
\expandafter\def\csname R@tworoom-gcbc-25\endcsname{100}
\expandafter\def\csname R@tworoom-gcbc-50\endcsname{98}
\expandafter\def\csname R@tworoom-gcbc-75\endcsname{100}
\expandafter\def\csname R@tworoom-gcbc-x\endcsname{99}
\expandafter\def\csname R@tworoom-gciql-25\endcsname{61}
\expandafter\def\csname R@tworoom-gciql-50\endcsname{51}
\expandafter\def\csname R@tworoom-gciql-75\endcsname{37}
\expandafter\def\csname R@tworoom-gciql-x\endcsname{46}
\expandafter\def\csname R@tworoom-gcivl-25\endcsname{99}
\expandafter\def\csname R@tworoom-gcivl-50\endcsname{90}
\expandafter\def\csname R@tworoom-gcivl-75\endcsname{81}
\expandafter\def\csname R@tworoom-gcivl-x\endcsname{86}
\expandafter\def\csname R@tworoom-hilp-25\endcsname{98}
\expandafter\def\csname R@tworoom-hilp-50\endcsname{95}
\expandafter\def\csname R@tworoom-hilp-75\endcsname{87}
\expandafter\def\csname R@tworoom-hilp-x\endcsname{89}
\expandafter\def\csname R@tworoom-ours-25\endcsname{96}
\expandafter\def\csname R@tworoom-ours-50\endcsname{93}
\expandafter\def\csname R@tworoom-ours-75\endcsname{93}
\expandafter\def\csname R@tworoom-ours-x\endcsname{99}
\expandafter\def\csname R@tworoom-pldm-25\endcsname{98}
\expandafter\def\csname R@tworoom-pldm-50\endcsname{75}
\expandafter\def\csname R@tworoom-pldm-75\endcsname{50}
\expandafter\def\csname R@tworoom-pldm-x\endcsname{81}
\expandafter\def\csname R@tworoom-released-25\endcsname{88}
\expandafter\def\csname R@tworoom-released-50\endcsname{54}
\expandafter\def\csname R@tworoom-released-75\endcsname{31}
\expandafter\def\csname R@tworoom-released-x\endcsname{61}
\expandafter\def\csname R@tworoom-relmin-25\endcsname{99}
\expandafter\def\csname R@tworoom-relmin-50\endcsname{81}
\expandafter\def\csname R@tworoom-relmin-75\endcsname{62}
\expandafter\def\csname R@tworoom-relmin-x\endcsname{82}
\expandafter\def\csname R@wp-gcbc-100\endcsname{80}
\expandafter\def\csname R@wp-gcbc-150\endcsname{58}
\expandafter\def\csname R@wp-gcbc-200\endcsname{38}
\expandafter\def\csname R@wp-gcbc-50\endcsname{94}
\expandafter\def\csname R@wp-gcbc-x\endcsname{54}
\expandafter\def\csname R@wp-gcbcg-100\endcsname{86}
\expandafter\def\csname R@wp-gcbcg-150\endcsname{58}
\expandafter\def\csname R@wp-gcbcg-200\endcsname{34}
\expandafter\def\csname R@wp-gcbcg-50\endcsname{94}
\expandafter\def\csname R@wp-gcbcg-x\endcsname{54}
\makeatother


==> tables/numbers_pushtdist.tex <==
% generated by figs/scripts/fig_pusht_distance.py; do not edit
\makeatletter
\providecommand{\Ed}[1]{\csname Ed@#1\endcsname}
\expandafter\def\csname Ed@ours-50\endcsname{85}
\expandafter\def\csname Ed@ours-50-n\endcsname{3}
\expandafter\def\csname Ed@ours-75\endcsname{80}
\expandafter\def\csname Ed@ours-75-n\endcsname{3}
\expandafter\def\csname Ed@ours-100\endcsname{71}
\expandafter\def\csname Ed@ours-100-n\endcsname{3}
\expandafter\def\csname Ed@ours-150\endcsname{71}
\expandafter\def\csname Ed@ours-150-n\endcsname{3}
\expandafter\def\csname Ed@ours-200\endcsname{71}
\expandafter\def\csname Ed@ours-200-n\endcsname{2}
\expandafter\def\csname Ed@ap-50\endcsname{82}
\expandafter\def\csname Ed@ap-50-n\endcsname{1}
\expandafter\def\csname Ed@ap-75\endcsname{66}
\expandafter\def\csname Ed@ap-75-n\endcsname{1}
\expandafter\def\csname Ed@ap-100\endcsname{86}
\expandafter\def\csname Ed@ap-100-n\endcsname{1}
\expandafter\def\csname Ed@ap-150\endcsname{65}
\expandafter\def\csname Ed@ap-150-n\endcsname{3}
\expandafter\def\csname Ed@ap-200\endcsname{56}
\expandafter\def\csname Ed@ap-200-n\endcsname{2}
\expandafter\def\csname Ed@ngc-50\endcsname{59}
\expandafter\def\csname Ed@ngc-50-n\endcsname{2}
\expandafter\def\csname Ed@ngc-100\endcsname{23}
\expandafter\def\csname Ed@ngc-100-n\endcsname{2}
\expandafter\def\csname Ed@ngc-150\endcsname{11}
\expandafter\def\csname Ed@ngc-150-n\endcsname{2}
\expandafter\def\csname Ed@ngc-200\endcsname{4}
\expandafter\def\csname Ed@ngc-200-n\endcsname{2}
\expandafter\def\csname Ed@metro-50\endcsname{72}
\expandafter\def\csname Ed@metro-50-n\endcsname{3}
\expandafter\def\csname Ed@metro-75\endcsname{54}
\expandafter\def\csname Ed@metro-75-n\endcsname{3}
\expandafter\def\csname Ed@metro-150\endcsname{33}
\expandafter\def\csname Ed@metro-150-n\endcsname{3}
\expandafter\def\csname Ed@metro-200\endcsname{27}
\expandafter\def\csname Ed@metro-200-n\endcsname{2}
\expandafter\def\csname Ed@lewm-50\endcsname{41}
\expandafter\def\csname Ed@lewm-50-n\endcsname{2}
\expandafter\def\csname Ed@lewm-75\endcsname{21}
\expandafter\def\csname Ed@lewm-75-n\endcsname{2}
\expandafter\def\csname Ed@lewm-100\endcsname{17}
\expandafter\def\csname Ed@lewm-100-n\endcsname{2}
\expandafter\def\csname Ed@lewm-150\endcsname{5}
\expandafter\def\csname Ed@lewm-150-n\endcsname{2}
\expandafter\def\csname Ed@lewm-200\endcsname{2}
\expandafter\def\csname Ed@lewm-200-n\endcsname{2}
\makeatother


==> tables/numbers_r2.tex <==
% generated by figs/scripts/make_tables_r2.py -- do not edit
\makeatletter
\newcommand{\Q}[1]{\@ifundefined{Q@#1}{\pendnum{#1}}{\csname Q@#1\endcsname}}
\expandafter\def\csname Q@apd-loss-pmm-200\endcsname{50}
\expandafter\def\csname Q@apd-pml-200-0.5\endcsname{17}
\expandafter\def\csname Q@apd-pml-200-1\endcsname{16}
\expandafter\def\csname Q@apd-pml-200-2\endcsname{17}
\expandafter\def\csname Q@apd-pml-200-ours\endcsname{73}
\expandafter\def\csname Q@apd-pml-400-0.5\endcsname{11}
\expandafter\def\csname Q@apd-pml-400-1\endcsname{12}
\expandafter\def\csname Q@apd-pml-400-2\endcsname{14}
\expandafter\def\csname Q@apd-pml-400-ours\endcsname{87}
\expandafter\def\csname Q@apd-pmm-100-0.25\endcsname{47}
\expandafter\def\csname Q@apd-pmm-100-0.5\endcsname{59}
\expandafter\def\csname Q@apd-pmm-100-0.75\endcsname{95}
\expandafter\def\csname Q@apd-pmm-100-1\endcsname{92}
\expandafter\def\csname Q@apd-pmm-100-1.5\endcsname{74}
\expandafter\def\csname Q@apd-pmm-100-2\endcsname{50}
\expandafter\def\csname Q@apd-pmm-100-3\endcsname{15}
\expandafter\def\csname Q@apd-pmm-100-ours\endcsname{89}
\expandafter\def\csname Q@apd-pmm-200-0.25\endcsname{29}
\expandafter\def\csname Q@apd-pmm-200-0.5\endcsname{31}
\expandafter\def\csname Q@apd-pmm-200-0.75\endcsname{54}
\expandafter\def\csname Q@apd-pmm-200-1\endcsname{81}
\expandafter\def\csname Q@apd-pmm-200-1.5\endcsname{70}
\expandafter\def\csname Q@apd-pmm-200-2\endcsname{48}
\expandafter\def\csname Q@apd-pmm-200-3\endcsname{11}
\expandafter\def\csname Q@apd-pmm-200-ours\endcsname{87}
\expandafter\def\csname Q@apd-tworoom-75-0.25\endcsname{36}
\expandafter\def\csname Q@apd-tworoom-75-0.5\endcsname{83}
\expandafter\def\csname Q@apd-tworoom-75-1\endcsname{96}
\expandafter\def\csname Q@apd-tworoom-75-2\endcsname{96}
\expandafter\def\csname Q@apd-tworoom-75-3\endcsname{2}
\expandafter\def\csname Q@apd-tworoom-75-ours\endcsname{94}
\expandafter\def\csname Q@apd-worst-pmm-200\endcsname{11}
\expandafter\def\csname Q@bud-gcbc1-100\endcsname{83}
\expandafter\def\csname Q@bud-gcbc1-150\endcsname{54}
\expandafter\def\csname Q@bud-gcbc1-200\endcsname{51}
\expandafter\def\csname Q@bud-gcbc1-50\endcsname{93}
\expandafter\def\csname Q@bud-gcbc1-x\endcsname{51}
\expandafter\def\csname Q@bud-gcbc4-100\endcsname{88}
\expandafter\def\csname Q@bud-gcbc4-150\endcsname{68}
\expandafter\def\csname Q@bud-gcbc4-200\endcsname{58}
\expandafter\def\csname Q@bud-gcbc4-50\endcsname{98}
\expandafter\def\csname Q@bud-gcbc4-x\endcsname{59}
\expandafter\def\csname Q@bud-gcivl1-100\endcsname{4}
\expandafter\def\csname Q@bud-gcivl1-150\endcsname{2}
\expandafter\def\csname Q@bud-gcivl1-200\endcsname{0}
\expandafter\def\csname Q@bud-gcivl1-50\endcsname{30}
\expandafter\def\csname Q@bud-gcivl1-x\endcsname{16}
\expandafter\def\csname Q@bud-gcivl4-100\endcsname{2}
\expandafter\def\csname Q@bud-gcivl4-150\endcsname{0}
\expandafter\def\csname Q@bud-gcivl4-200\endcsname{0}
\expandafter\def\csname Q@bud-gcivl4-50\endcsname{30}
\expandafter\def\csname Q@bud-gcivl4-x\endcsname{12}
\expandafter\def\csname Q@bud-pldm5-ap-100\endcsname{38}
\expandafter\def\csname Q@bud-pldm5-ap-200\endcsname{9}
\expandafter\def\csname Q@bud-pldm5-ap-x\endcsname{29}
\expandafter\def\csname Q@bud-pldm5-ours-100\endcsname{33}
\expandafter\def\csname Q@bud-pldm5-ours-200\endcsname{7}
\expandafter\def\csname Q@bud-pldm5-ours-x\endcsname{29}
\expandafter\def\csname Q@bud-pldm5-released-100\endcsname{8}
\expandafter\def\csname Q@bud-pldm5-released-200\endcsname{1}
\expandafter\def\csname Q@bud-pldm5-released-50\endcsname{28}
\expandafter\def\csname Q@bud-pldm5-released-x\endcsname{20}
\expandafter\def\csname Q@bud-pldm5-relmin-100\endcsname{10}
\expandafter\def\csname Q@bud-pldm5-relmin-200\endcsname{1}
\expandafter\def\csname Q@drop-pmm-100\endcsname{79}
\expandafter\def\csname Q@drop-pmm-200\endcsname{83}
\expandafter\def\csname Q@fa-pmm-gah5\endcsname{85}
\expandafter\def\csname Q@fa-pmm-ours\endcsname{87}
\expandafter\def\csname Q@fa-pmm-released\endcsname{12}
\expandafter\def\csname Q@fa-pmm-relmin\endcsname{9}
\expandafter\def\csname Q@fa-tworoom-gah5\endcsname{66}
\expandafter\def\csname Q@fa-tworoom-ours\endcsname{94}
\expandafter\def\csname Q@fa-tworoom-released\endcsname{32}
\expandafter\def\csname Q@fa-tworoom-relmin\endcsname{61}
\expandafter\def\csname Q@fail-d200-dmax\endcsname{2.2}
\expandafter\def\csname Q@fail-d200-dmin\endcsname{1.4}
\expandafter\def\csname Q@fail-d200-failed\endcsname{4}
\expandafter\def\csname Q@fail-d200-n\endcsname{50}
\expandafter\def\csname Q@fail-d200-nearanchor\endcsname{4}
\expandafter\def\csname Q@fail-d200-noanchor\endcsname{0}
\expandafter\def\csname Q@fail-d200-stuck\endcsname{0}
\expandafter\def\csname Q@fail-x-dmax\endcsname{1.1}
\expandafter\def\csname Q@fail-x-dmin\endcsname{1.1}
\expandafter\def\csname Q@fail-x-failed\endcsname{1}
\expandafter\def\csname Q@fail-x-n\endcsname{50}
\expandafter\def\csname Q@fail-x-nearanchor\endcsname{1}
\expandafter\def\csname Q@fail-x-noanchor\endcsname{0}
\expandafter\def\csname Q@fail-x-stuck\endcsname{0}
\expandafter\def\csname Q@frac-0.01-ap\endcsname{67}
\expandafter\def\csname Q@frac-0.01-ap_x\endcsname{64}
\expandafter\def\csname Q@frac-0.01-ours\endcsname{63}
\expandafter\def\csname Q@frac-0.01-ours_x\endcsname{86}
\expandafter\def\csname Q@frac-0.02-ap\endcsname{69}
\expandafter\def\csname Q@frac-0.02-ap_x\endcsname{68}
\expandafter\def\csname Q@frac-0.02-ours\endcsname{80}
\expandafter\def\csname Q@frac-0.02-ours_x\endcsname{73}
\expandafter\def\csname Q@frac-0.05-ap\endcsname{75}
\expandafter\def\csname Q@frac-0.05-ap_x\endcsname{65}
\expandafter\def\csname Q@frac-0.05-ours\endcsname{78}
\expandafter\def\csname Q@frac-0.05-ours_x\endcsname{86}
\expandafter\def\csname Q@frac-0.1-ap\endcsname{72}
\expandafter\def\csname Q@frac-0.1-ours\endcsname{79}
\expandafter\def\csname Q@frac-0.25-ap\endcsname{81}
\expandafter\def\csname Q@frac-0.25-ours\endcsname{83}
\expandafter\def\csname Q@frac-0.5-ap\endcsname{83}
\expandafter\def\csname Q@frac-0.5-ours\endcsname{84}
\expandafter\def\csname Q@frac-1-ap\endcsname{81}
\expandafter\def\csname Q@frac-1-ap_x\endcsname{73}
\expandafter\def\csname Q@frac-1-ours\endcsname{86}
\expandafter\def\csname Q@frac-1-ours_x\endcsname{94}
\expandafter\def\csname Q@mw-demo-mean\endcsname{90}
\expandafter\def\csname Q@mw-demo-n\endcsname{72}
\expandafter\def\csname Q@mw-demo-solved\endcsname{65}
\expandafter\def\csname Q@pml-ap-100\endcsname{11}
\expandafter\def\csname Q@pml-ap-200\endcsname{16}
\expandafter\def\csname Q@pml-ap-400\endcsname{12}
\expandafter\def\csname Q@pml-ap-50\endcsname{17}
\expandafter\def\csname Q@pml-ap-x\endcsname{6}
\expandafter\def\csname Q@pml-gainmax\endcsname{79}
\expandafter\def\csname Q@pml-gainmin\endcsname{48}
\expandafter\def\csname Q@pml-nedges-m\endcsname{2.3}
\expandafter\def\csname Q@pml-nodes-k\endcsname{200}
\expandafter\def\csname Q@pml-ours-100\endcsname{63}
\expandafter\def\csname Q@pml-ours-200\endcsname{73}
\expandafter\def\csname Q@pml-ours-400\endcsname{87}
\expandafter\def\csname Q@pml-ours-50\endcsname{62}
\expandafter\def\csname Q@pml-ours-x\endcsname{66}
\expandafter\def\csname Q@pml-released-100\endcsname{15}
\expandafter\def\csname Q@pml-released-200\endcsname{13}
\expandafter\def\csname Q@pml-released-400\endcsname{8}
\expandafter\def\csname Q@pml-released-50\endcsname{14}
\expandafter\def\csname Q@pml-released-x\endcsname{5}
\expandafter\def\csname Q@pml-relmin-100\endcsname{28}
\expandafter\def\csname Q@pml-relmin-200\endcsname{23}
\expandafter\def\csname Q@pml-relmin-400\endcsname{26}
\expandafter\def\csname Q@pml-relmin-50\endcsname{44}
\expandafter\def\csname Q@pml-relmin-x\endcsname{17}
\expandafter\def\csname Q@pml-sd_ap-100\endcsname{15}
\expandafter\def\csname Q@pml-sd_ap-200\endcsname{17}
\expandafter\def\csname Q@pml-sd_ap-400\endcsname{12}
\expandafter\def\csname Q@pml-sd_ap-x\endcsname{10}
\expandafter\def\csname Q@pml-sd_ours-100\endcsname{61}
\expandafter\def\csname Q@pml-sd_ours-200\endcsname{68}
\expandafter\def\csname Q@pml-sd_ours-400\endcsname{87}
\expandafter\def\csname Q@pml-sd_ours-x\endcsname{56}
\expandafter\def\csname Q@pml-tedges-k\endcsname{199}
\expandafter\def\csname Q@st-budget-400-ap\endcsname{73}
\expandafter\def\csname Q@st-budget-400-ours\endcsname{94}
\expandafter\def\csname Q@st-budget-600-ap\endcsname{75}
\expandafter\def\csname Q@st-budget-600-ours\endcsname{99}
\expandafter\def\csname Q@st-budget-800-ap\endcsname{72}
\expandafter\def\csname Q@st-budget-800-ours\endcsname{99}
\expandafter\def\csname Q@st-kid-pmm-ap\endcsname{22}
\expandafter\def\csname Q@st-kid-pmm-ours\endcsname{65}
\expandafter\def\csname Q@st-kid-tworoom-ap\endcsname{75}
\expandafter\def\csname Q@st-kid-tworoom-ours\endcsname{74}
\expandafter\def\csname Q@st-kidref-pmm-ap\endcsname{81}
\expandafter\def\csname Q@st-kidref-pmm-ours\endcsname{86}
\expandafter\def\csname Q@st-kidref-tworoom-ap\endcsname{96}
\expandafter\def\csname Q@st-kidref-tworoom-ours\endcsname{93}
\expandafter\def\csname Q@st-reacher-ap\endcsname{40}
\expandafter\def\csname Q@st-reacher-ours\endcsname{62}
\expandafter\def\csname Q@st-reacher-relmin\endcsname{78}
\expandafter\def\csname Q@sw-10-100\endcsname{60}
\expandafter\def\csname Q@sw-10-150\endcsname{46}
\expandafter\def\csname Q@sw-3-100\endcsname{56}
\expandafter\def\csname Q@sw-3-150\endcsname{48}
\expandafter\def\csname Q@td-cube-rho10\endcsname{0.61}
\expandafter\def\csname Q@td-cube-rho3\endcsname{0.84}
\expandafter\def\csname Q@td-cube-rho6\endcsname{0.68}
\expandafter\def\csname Q@td-cube-spall\endcsname{0.44}
\expandafter\def\csname Q@td-cube-sploc\endcsname{0.54}
\expandafter\def\csname Q@td-pmm-rho10\endcsname{0.32}
\expandafter\def\csname Q@td-pmm-rho3\endcsname{0.98}
\expandafter\def\csname Q@td-pmm-rho6\endcsname{0.66}
\expandafter\def\csname Q@td-pmm-spall\endcsname{0.27}
\expandafter\def\csname Q@td-pmm-sploc\endcsname{0.82}
\expandafter\def\csname Q@td-pmm-worm\endcsname{0.0}
\expandafter\def\csname Q@td-pusht-rho10\endcsname{0.60}
\expandafter\def\csname Q@td-pusht-rho3\endcsname{0.96}
\expandafter\def\csname Q@td-pusht-rho6\endcsname{0.83}
\expandafter\def\csname Q@td-pusht-spall\endcsname{0.48}
\expandafter\def\csname Q@td-pusht-sploc\endcsname{0.69}
\expandafter\def\csname Q@td-pusht-worm\endcsname{0.2}
\expandafter\def\csname Q@td-reacher-rho10\endcsname{0.52}
\expandafter\def\csname Q@td-reacher-rho3\endcsname{0.74}
\expandafter\def\csname Q@td-reacher-rho6\endcsname{0.59}
\expandafter\def\csname Q@td-reacher-spall\endcsname{0.33}
\expandafter\def\csname Q@td-reacher-sploc\endcsname{0.43}
\expandafter\def\csname Q@td-tworoom-rho10\endcsname{0.56}
\expandafter\def\csname Q@td-tworoom-rho3\endcsname{0.62}
\expandafter\def\csname Q@td-tworoom-rho6\endcsname{0.56}
\expandafter\def\csname Q@td-tworoom-spall\endcsname{0.27}
\expandafter\def\csname Q@td-tworoom-sploc\endcsname{0.26}
\expandafter\def\csname Q@td-tworoom-worm\endcsname{0.0}
\expandafter\def\csname Q@time-build-s\endcsname{51}
\expandafter\def\csname Q@time-dijkstra-ms\endcsname{9}
\expandafter\def\csname Q@time-ga\endcsname{1.8}
\expandafter\def\csname Q@time-ga-sr\endcsname{80}
\expandafter\def\csname Q@time-released\endcsname{1.5}
\expandafter\def\csname Q@time-released-sr\endcsname{30}
\expandafter\def\csname Q@time-relmin\endcsname{2.6}
\expandafter\def\csname Q@time-relmin-sr\endcsname{20}
\expandafter\def\csname Q@wp2-gcbc-100\endcsname{83}
\expandafter\def\csname Q@wp2-gcbc-200\endcsname{55}
\expandafter\def\csname Q@wp2-gcbc-x\endcsname{51}
\expandafter\def\csname Q@wp2-gcbcg-100\endcsname{82}
\expandafter\def\csname Q@wp2-gcbcg-200\endcsname{43}
\expandafter\def\csname Q@wp2-gcbcg-ratio\endcsname{8.2}
\expandafter\def\csname Q@wp2-gcbcg-reach\endcsname{0.4}
\expandafter\def\csname Q@wp2-gcbcg-x\endcsname{57}
\expandafter\def\csname Q@wp2-gcbcg2-100\endcsname{71}
\expandafter\def\csname Q@wp2-gcbcg2-200\endcsname{25}
\expandafter\def\csname Q@wp2-gcbcg2-ratio\endcsname{1.4}
\expandafter\def\csname Q@wp2-gcbcg2-reach\endcsname{37.0}
\expandafter\def\csname Q@wp2-gcbcg2-x\endcsname{40}
\expandafter\def\csname Q@wp2-ours-200\endcsname{87}
\makeatother


==> tables/numbers_stats.tex <==
% generated by figs/scripts/stats.py -- do not edit
\makeatletter
\newcommand{\Sx}[1]{\@ifundefined{S@#1}{\textbf{??#1}}{\csname S@#1\endcsname}}
\expandafter\def\csname S@hwmin\endcsname{3}
\expandafter\def\csname S@hwmax\endcsname{8}
\expandafter\def\csname S@p-pointmaze-m-d-50-lewm-planner\endcsname{<0.001}
\expandafter\def\csname S@p-pointmaze-m-d-50-lewm-min-over-plan\endcsname{<0.001}
\expandafter\def\csname S@p-pointmaze-m-d-100-lewm-planner\endcsname{<0.001}
\expandafter\def\csname S@p-pointmaze-m-d-100-lewm-min-over-plan\endcsname{<0.001}
\expandafter\def\csname S@p-pointmaze-m-d-150-lewm-planner\endcsname{<0.001}
\expandafter\def\csname S@p-pointmaze-m-d-150-lewm-min-over-plan\endcsname{<0.001}
\expandafter\def\csname S@p-pointmaze-m-d-200-lewm-planner\endcsname{<0.001}
\expandafter\def\csname S@p-pointmaze-m-d-200-lewm-min-over-plan\endcsname{<0.001}
\expandafter\def\csname S@p-two-room-d-25-lewm-planner\endcsname{0.004}
\expandafter\def\csname S@p-two-room-d-25-lewm-min-over-plan\endcsname{0.219}
\expandafter\def\csname S@p-two-room-d-50-lewm-planner\endcsname{<0.001}
\expandafter\def\csname S@p-two-room-d-50-lewm-min-over-plan\endcsname{0.001}
\expandafter\def\csname S@p-two-room-d-75-lewm-planner\endcsname{<0.001}
\expandafter\def\csname S@p-two-room-d-75-lewm-min-over-plan\endcsname{<0.001}
\expandafter\def\csname S@p-pointmaze-m-stitched-lewm-planner\endcsname{<0.001}
\expandafter\def\csname S@p-pointmaze-m-stitched-lewm-min-over-plan\endcsname{<0.001}
\expandafter\def\csname S@p-two-room-stitched-lewm-planner\endcsname{<0.001}
\expandafter\def\csname S@p-two-room-stitched-lewm-min-over-plan\endcsname{<0.001}
\expandafter\def\csname S@p-pointmaze-l-d-50-lewm-planner\endcsname{<0.001}
\expandafter\def\csname S@p-pointmaze-l-d-50-lewm-min-over-plan\endcsname{0.008}
\expandafter\def\csname S@p-pointmaze-l-d-100-lewm-planner\endcsname{<0.001}
\expandafter\def\csname S@p-pointmaze-l-d-100-lewm-min-over-plan\endcsname{<0.001}
\expandafter\def\csname S@p-pointmaze-l-d-200-lewm-planner\endcsname{<0.001}
\expandafter\def\csname S@p-pointmaze-l-d-200-lewm-min-over-plan\endcsname{<0.001}
\expandafter\def\csname S@p-pointmaze-l-d-400-lewm-planner\endcsname{<0.001}
\expandafter\def\csname S@p-pointmaze-l-d-400-lewm-min-over-plan\endcsname{<0.001}
\expandafter\def\csname S@p-pointmaze-l-stitched-lewm-planner\endcsname{<0.001}
\expandafter\def\csname S@p-pointmaze-l-stitched-lewm-min-over-plan\endcsname{<0.001}
\expandafter\def\csname S@p-pointmaze-m-d-100-gcbc\endcsname{0.229}
\expandafter\def\csname S@p-pointmaze-m-d-200-gcbc\endcsname{<0.001}
\expandafter\def\csname S@p-pointmaze-m-stitched-gcbc\endcsname{<0.001}
\expandafter\def\csname S@p-random-play-graph-d-150-expert-graph\endcsname{1.000}
\expandafter\def\csname S@p-random-play-graph-d-200-expert-graph\endcsname{0.200}
\expandafter\def\csname S@p-graph-gcbc-d-100-gcbc\endcsname{0.774}
\expandafter\def\csname S@p-graph-gcbc-d-200-gcbc\endcsname{0.003}
\makeatother


==> tables/pldm_rows.tex <==
PLDM planner & 98 & 75 & 50 & 81 && 17 & 3 & 28 \\
+ min-over-plan & 100 & 85 & 62 & -- && 12 & 4 & -- \\
\rowcolor{pactrow}\textbf{+ graph anchors (ours)} & 95 & 98 & 97 & 99 && 28 & 4 & 28 \\


==> tables/pml_rows.tex <==
LeWM planner & 14 & 15 & 13 & 8 & 5 \\
LeWM + min-over-plan & 44 & 28 & 23 & 26 & 17 \\
\rowcolor{pactrow}Graph anchors, navigate data (training data) & 62 & 63 & 73 & 87 & 66 \\
Graph anchors, stitch dataset & -- & 61 & 68 & 87 & 56 \\


==> tables/published_rows.tex <==
Push-T & 96 & 78 & 74 & 75 & 20 & 33 \\
Two-Room & 87 & 97 & 100 & 100 & 100 & 100 \\
Reacher & 86 & 78 & 79 & -- & -- & -- \\
OGBench-Cube & 74 & 65 & 86 & 84 & 64 & 56 \\


==> tables/rand_rows.tex <==
Graph anchors, expert graph & 90 & 88 & 91 & 86 & 94 \\
Graph anchors, random-play graph & 95 & 90 & 87 & 90 & 95 \\


==> tables/retrain_rows.tex <==
\multicolumn{6}{@{}l}{\emph{Original model (Table 1)}} \\
\quad LeWM & 14 & 15 & 13 & 8 & 5 \\
\quad LeWM + min-over-plan & 44 & 28 & 23 & 26 & 17 \\
\quad AP (our re-implementation) & 17 & 11 & 16 & 12 & 6 \\
\rowcolor{oursrow}\quad Graph Anchors, navigation setting & 62 & 63 & 73 & 87 & 66 \\
\multicolumn{6}{@{}l}{\emph{Second training run}} \\
\quad LeWM & 14 & 11 & 10 & 4 & 8 \\
\quad LeWM + min-over-plan & 38 & 25 & 24 & 20 & 21 \\
\quad AP (our re-implementation) & 31 & 16 & 17 & 18 & 9 \\
\rowcolor{oursrow}\quad Graph Anchors, navigation setting & 47 & 43 & 58 & 76 & 45 \\
\quad Graph Anchors, contact setting & -- & -- & -- & 13 & 9 \\


==> tables/seed_rows.tex <==
Push-T & LeWM planner & 25: 88, 50: 32/50, 75: 24/18, 100: 18/16, 150: 2/8 \\
Push-T & LeWM + min-over-plan & 25: 94, 50: 48/62, 75: 38/28, 100: 22/12, 150: 8/10 \\
Push-T & Graph anchors (ours) & 50: 64/66, 75: 50/50, 100: 38/42, 150: 28/32 \\
Two-Room & LeWM planner & 25: 88/84, 50: 52/50, 75: 28/32 \\
Two-Room & LeWM + min-over-plan & 25: 98/98, 50: 76/86, 75: 50/68 \\
Two-Room & Graph anchors (ours) & 25: 92/96, 50: 92/94, 75: 94/92 \\
PointMaze-M & LeWM planner & 50: 38/50, 100: 24/22, 150: 10/12, 200: 16/12 \\
PointMaze-M & LeWM + min-over-plan & 50: 66/68, 100: 30/40, 150: 12/20, 200: 14/6 \\
PointMaze-M & Graph anchors (ours) & 50: 90/90, 100: 84/92, 150: 88/94, 200: 92/80 \\
OGBench-Cube & LeWM planner & 25: 70, 50: 64, 100: 50, 150: 20 \\
OGBench-Cube & LeWM + min-over-plan & 25: 68, 50: 60, 100: 56, 150: 20 \\
OGBench-Cube & Graph anchors (ours) & 25: 70, 50: 56, 100: 60, 150: 20 \\
Reacher & LeWM planner & 25: 60, 50: 74, 100: 62, 150: 66 \\
Reacher & LeWM + min-over-plan & 25: 82, 50: 80, 100: 78, 150: 74 \\
Reacher & Graph anchors (ours) & 25: 60, 50: 60, 100: 64, 150: 64 \\


==> tables/seedx_grid.tex <==
% generated by figs/scripts/seedx_grid.py; do not edit
\multicolumn{6}{@{}l}{\textbf{Push-T}} \\
 & $d{=}25$ & $d{=}50$ & $d{=}75$ & $d{=}100$ & $d{=}150$ \\
\midrule
LeWM & 88/90/88 & 32/50 & 24/18 & 18/16 & 2/8 \\
LeWM + min-over-plan & 94/90/88 & 48/62 & 38/28 & 22/12 & 8/10 \\
Graph Anchors & 88/82/76 & 64/66 & 50/50 & 38/42 & 28/32 \\
GCBC & 52/28 & 20/12 & 12/4 & 10/12 & 6/4 \\
GCIVL & 4/0 & 2/2 & 0/0 & 0/0 & 0/0 \\
GCIQL & 0/0 & 0/0 & 0/0 & 0/0 & 0/0 \\
HILP & 6/2 & 0/0 & 0/0 & 0/0 & 0/0 \\
\addlinespace[4pt]
\multicolumn{6}{@{}l}{\textbf{Two-Room (stitched: budget 200)}} \\
 & $d{=}25$ & $d{=}50$ & $d{=}75$ & stitched &  \\
\midrule
LeWM & 88/84/92 & 52/50/60 & 28/32/34 & 56/68/60 &  \\
LeWM + min-over-plan & 98/98/100 & 76/86/82 & 50/68/68 & 84/78/84 &  \\
Graph Anchors & 92/96/100 & 92/94/94 & 94/92/94 & 100/98/98 &  \\
GCBC & 100 & 98 & 100 & 98/100 &  \\
GCIVL & 100/100/96 & 90/90/90 & 84/80/80 & 82/90 &  \\
GCIQL & 62/60/62 & 62/40/52 & 38/32/40 & 46/46 &  \\
HILP & 98/98/98 & 96/96/94 & 84/86/90 & 88/90 &  \\
PLDM planner & 100/96 & 76/74 & 46/54 & 80/82 &  \\
PLDM + min-over-plan & 100/100 & 88/82 & 62/62 &  &  \\
PLDM + graph anchors & 94/96 & 96/100 & 98/96 & 100/98 &  \\
\addlinespace[4pt]
\multicolumn{6}{@{}l}{\textbf{PointMaze-Medium (stitched: budget 400)}} \\
 & $d{=}50$ & $d{=}100$ & $d{=}150$ & $d{=}200$ & stitched \\
\midrule
LeWM & 38/50/62 & 24/22/30 & 10/12/16 & 16/12/12 & 46/32 \\
LeWM + min-over-plan & 66/68/76 & 30/40/30 & 12/20/18 & 14/6/16 & 44/38 \\
Graph Anchors & 90/90/94 & 84/92/90 & 88/94/82 & 92/80/82 & 98/90/96 \\
GCBC & 92/94 & 84/80/82/86/82 & 50/58 & 52/38/54/56/54 & 48/46/56/52/46/60/46 \\
GCIVL & 30 & 4 & 2 & 0 & 16/16 \\
GCIQL & 32/40/30 & 6/4/2 & 0/0/0 & 2/0/0 & 14/10 \\
HILP & 28/36/32 & 4/4/0 & 0/2/0 & 2/0/0 & 18/18 \\
PLDM planner & 26/34 & 20/14/16/18 & 4/4 & 6/0/6/0 & 30/24/32/26 \\
PLDM + min-over-plan & 50/52 & 12/8/16/14 & 2/6 & 8/4/2/4 & 26/28 \\
PLDM + graph anchors & 52/66 & 30/24/30/28 & 8/10 & 4/2/4/4 & 30/30/30/24 \\
\addlinespace[4pt]
\multicolumn{6}{@{}l}{\textbf{PointMaze-Large (stitched: budget 400)}} \\
 & $d{=}50$ & $d{=}100$ & $d{=}200$ & $d{=}400$ & stitched \\
\midrule
LeWM & 16/12 & 20/10 & 10/16 & 8/8 & 4/6 \\
LeWM + min-over-plan & 50/38 & 30/26 & 20/26 & 30/22 & 18/16 \\
Graph Anchors & 66/58 & 58/68 & 76/70 & 88/86 & 70/62 \\
GCBC & 24/42 & 22/28 & 16/20 & 20/16 & 16/18 \\
GCIVL & 8/10 & 10/6 & 10/8 & 2/0 & 2/4 \\
GCIQL & 8/10 & 10/6 & 10/8 & 2/4 & 2/4 \\
HILP & 12/12 & 16/10 & 14/18 & 10/8 & 6/14 \\
\addlinespace[4pt]
\multicolumn{6}{@{}l}{\textbf{OGBench-Cube}} \\
 & $d{=}25$ & $d{=}50$ & $d{=}100$ & $d{=}150$ &  \\
\midrule
LeWM & 70 & 64 & 50 & 20 &  \\
LeWM + min-over-plan & 68 & 60 & 56 & 20 &  \\
Graph Anchors & 70 & 56 & 60 & 20 &  \\
\addlinespace[4pt]
\multicolumn{6}{@{}l}{\textbf{Reacher}} \\
 & $d{=}25$ & $d{=}50$ & $d{=}100$ & $d{=}150$ &  \\
\midrule
LeWM & 60 & 74 & 62 & 66 &  \\
LeWM + min-over-plan & 82 & 80 & 78 & 74 &  \\
Graph Anchors & 60 & 60 & 64 & 64 &  \\



==> tables/seedx_rows.tex <==
Push-T & LeWM planner & 25: 88, 50: 32/50, 75: 24/18, 100: 18/16, 150: 2/8 \\
Push-T & LeWM + min-over-plan & 25: 94, 50: 48/62, 75: 38/28, 100: 22/12, 150: 8/10 \\
Push-T & Graph anchors  & 50: 64/66, 75: 50/50, 100: 38/42, 150: 28/32 \\
Two-Room & LeWM planner & 25: 88/84/92, 50: 52/50/60, 75: 28/32/34, st.: 56/68/60 \\
Two-Room & LeWM + min-over-plan & 25: 98/98/100, 50: 76/86/82, 75: 50/68/68, st.: 84/78/84 \\
Two-Room & Graph anchors  & 25: 92/96/100, 50: 92/94/94, 75: 94/92/94, st.: 100/98/98 \\
Two-Room & GCBC & 25: 100, 50: 98, 75: 100, st.: 98/100 \\
Two-Room & GCIVL & 25: 100/100/96, 50: 90/90/90, 75: 84/80/80, st.: 82/90 \\
PointMaze-M & LeWM planner & 50: 38/50/62, 100: 24/22/30, 150: 10/12/16, 200: 16/12/12, st.: 46/32 \\
PointMaze-M & LeWM + min-over-plan & 50: 66/68/76, 100: 30/40/30, 150: 12/20/18, 200: 14/6/16, st.: 44/38 \\
PointMaze-M & Graph anchors  & 50: 90/90/94, 100: 84/92/90, 150: 88/94/82, 200: 92/80/82, st.: 98/90/96 \\
PointMaze-M & GCBC & 50: 92/94, 100: 84/80/82/86/82, 150: 50/58, 200: 52/38/54/56/54, st.: 48/46/56/52/46/60/46 \\
PointMaze-M & GCIVL & 50: 30, 100: 4, 150: 2, 200: 0, st.: 16/16 \\
PointMaze-L & LeWM planner & 50: 16/12, 100: 20/10, 200: 10/16, 400: 8/8, st.: 4/6 \\
PointMaze-L & LeWM + min-over-plan & 50: 50/38, 100: 30/26, 200: 20/26, 400: 30/22, st.: 18/16 \\
PointMaze-L & Graph anchors  & 50: 66/58, 100: 58/68, 200: 76/70, 400: 88/86, st.: 70/62 \\
PointMaze-L & GCBC & 50: 24/42, 100: 22/28, 200: 16/20, 400: 20/16, st.: 16/18 \\
Two-Room & PLDM planner & 25: 100/96, 50: 76/74, 75: 46/54, st.: 80/82 \\
Two-Room & PLDM + min-over-plan & 25: 100/100, 50: 88/82, 75: 62/62 \\
Two-Room & PLDM + graph anchors & 25: 94/96, 50: 96/100, 75: 98/96, st.: 100/98 \\
PointMaze-M & PLDM planner & 100: 20/14/16/18, 200: 6/0/6/0, st.: 30/24/32/26 \\
PointMaze-M & PLDM + min-over-plan & 100: 12/8/16/14, 200: 8/4/2/4 \\
PointMaze-M & PLDM + graph anchors & 100: 30/24/30/28, 200: 4/2/4/4, st.: 30/30/30/24 \\
OGBench-Cube & LeWM planner & 25: 70, 50: 64, 100: 50, 150: 20 \\
OGBench-Cube & LeWM + min-over-plan & 25: 68, 50: 60, 100: 56, 150: 20 \\
OGBench-Cube & Graph anchors  & 25: 70, 50: 56, 100: 60, 150: 20 \\
Reacher & LeWM planner & 25: 60, 50: 74, 100: 62, 150: 66 \\
Reacher & LeWM + min-over-plan & 25: 82, 50: 80, 100: 78, 150: 74 \\
Reacher & Graph anchors  & 25: 60, 50: 60, 100: 64, 150: 64 \\


==> tables/span_rows.tex <==
Push-T & 50 & 8 & 32 & \textbf{64} & 54 & 50 \\
Push-T & 75 & 8 & -- & \textbf{50} & \textbf{50} & 42 \\
Push-T & 100 & -- & -- & 38 & \textbf{42} & 40 \\
Push-T & 150 & -- & -- & \textbf{28} & 22 & -- \\
Two-Room & 50 & -- & -- & \textbf{92} & \textbf{92} & -- \\
Two-Room & 75 & -- & -- & \textbf{94} & 82 & -- \\
PointMaze-M & 100 & -- & -- & \textbf{84} & 74 & -- \\
PointMaze-M & 150 & -- & -- & \textbf{88} & 74 & -- \\
PointMaze-M & 200 & -- & -- & \textbf{92} & 74 & -- \\


==> tables/spanx_rows.tex <==
PointMaze-M, $d{=}200$ & 57 & 77 & 83 & 75 & 35 \\
Two-Room, $d{=}75$ & 21 & 75 & 94 & 77 & 58 \\


==> tables/stats_rows.tex <==
PointMaze-M, $d{=}50$ & ours vs.\ LeWM planner & 3 & 150 & 91 / 50 & 66 / 4 & $<$0.001 \\
PointMaze-M, $d{=}50$ & ours vs.\ LeWM + min-over-plan & 3 & 150 & 91 / 70 & 37 / 5 & $<$0.001 \\
PointMaze-M, $d{=}100$ & ours vs.\ LeWM planner & 3 & 150 & 89 / 25 & 98 / 3 & $<$0.001 \\
PointMaze-M, $d{=}100$ & ours vs.\ LeWM + min-over-plan & 3 & 150 & 89 / 33 & 88 / 5 & $<$0.001 \\
PointMaze-M, $d{=}150$ & ours vs.\ LeWM planner & 3 & 150 & 88 / 13 & 114 / 1 & $<$0.001 \\
PointMaze-M, $d{=}150$ & ours vs.\ LeWM + min-over-plan & 3 & 150 & 88 / 17 & 110 / 3 & $<$0.001 \\
PointMaze-M, $d{=}200$ & ours vs.\ LeWM planner & 3 & 150 & 85 / 13 & 108 / 1 & $<$0.001 \\
PointMaze-M, $d{=}200$ & ours vs.\ LeWM + min-over-plan & 3 & 150 & 85 / 12 & 111 / 2 & $<$0.001 \\
Two-Room, $d{=}25$ & ours vs.\ LeWM planner & 3 & 150 & 96 / 88 & 14 / 2 & 0.004 \\
Two-Room, $d{=}25$ & ours vs.\ LeWM + min-over-plan & 3 & 150 & 96 / 99 & 1 / 5 & 0.219 \\
Two-Room, $d{=}50$ & ours vs.\ LeWM planner & 3 & 150 & 93 / 54 & 62 / 3 & $<$0.001 \\
Two-Room, $d{=}50$ & ours vs.\ LeWM + min-over-plan & 3 & 150 & 93 / 81 & 24 / 6 & 0.001 \\
Two-Room, $d{=}75$ & ours vs.\ LeWM planner & 3 & 150 & 93 / 31 & 94 / 1 & $<$0.001 \\
Two-Room, $d{=}75$ & ours vs.\ LeWM + min-over-plan & 3 & 150 & 93 / 62 & 50 / 3 & $<$0.001 \\
PointMaze-M, stitched & ours vs.\ LeWM planner & 2 & 100 & 97 / 39 & 58 / 0 & $<$0.001 \\
PointMaze-M, stitched & ours vs.\ LeWM + min-over-plan & 2 & 100 & 97 / 41 & 56 / 0 & $<$0.001 \\
Two-Room, stitched & ours vs.\ LeWM planner & 3 & 150 & 99 / 61 & 56 / 0 & $<$0.001 \\
Two-Room, stitched & ours vs.\ LeWM + min-over-plan & 3 & 150 & 99 / 82 & 26 / 1 & $<$0.001 \\
PointMaze-L, $d{=}50$ & ours vs.\ LeWM planner & 2 & 100 & 62 / 14 & 48 / 0 & $<$0.001 \\
PointMaze-L, $d{=}50$ & ours vs.\ LeWM + min-over-plan & 2 & 100 & 62 / 44 & 30 / 12 & 0.008 \\
PointMaze-L, $d{=}100$ & ours vs.\ LeWM planner & 2 & 100 & 63 / 15 & 49 / 1 & $<$0.001 \\
PointMaze-L, $d{=}100$ & ours vs.\ LeWM + min-over-plan & 2 & 100 & 63 / 28 & 39 / 4 & $<$0.001 \\
PointMaze-L, $d{=}200$ & ours vs.\ LeWM planner & 2 & 100 & 73 / 13 & 60 / 0 & $<$0.001 \\
PointMaze-L, $d{=}200$ & ours vs.\ LeWM + min-over-plan & 2 & 100 & 73 / 23 & 51 / 1 & $<$0.001 \\
PointMaze-L, $d{=}400$ & ours vs.\ LeWM planner & 2 & 100 & 87 / 8 & 79 / 0 & $<$0.001 \\
PointMaze-L, $d{=}400$ & ours vs.\ LeWM + min-over-plan & 2 & 100 & 87 / 26 & 62 / 1 & $<$0.001 \\
PointMaze-L, stitched & ours vs.\ LeWM planner & 2 & 100 & 66 / 5 & 61 / 0 & $<$0.001 \\
PointMaze-L, stitched & ours vs.\ LeWM + min-over-plan & 2 & 100 & 66 / 17 & 50 / 1 & $<$0.001 \\
PointMaze-M, $d{=}100$ & ours vs.\ GCBC & 3 & 150 & 89 / 83 & 21 / 13 & 0.229 \\
PointMaze-M, $d{=}200$ & ours vs.\ GCBC & 3 & 150 & 85 / 55 & 56 / 11 & $<$0.001 \\
PointMaze-M, stitched & ours vs.\ GCBC & 3 & 150 & 95 / 51 & 66 / 0 & $<$0.001 \\
Random-play graph, $d{=}150$ & random graph vs.\ expert graph & 3 & 150 & 87 / 88 & 14 / 15 & 1.000 \\
Random-play graph, $d{=}200$ & random graph vs.\ expert graph & 3 & 150 & 90 / 85 & 19 / 11 & 0.200 \\
Graph + GCBC, $d{=}100$ & GCBC + graph vs.\ GCBC & 3 & 150 & 82 / 83 & 5 / 7 & 0.774 \\
Graph + GCBC, $d{=}200$ & GCBC + graph vs.\ GCBC & 3 & 150 & 43 / 55 & 8 / 26 & 0.003 \\


==> tables/stress_rows.tex <==
Kidnapped mid-episode, PointMaze-M $d{=}200$ & 65 & 66/64 \\
Kidnapped mid-episode, Two-Room $d{=}75$ & 74 & 76/72 \\
Stitched goals, PointMaze-M, budget 400 & 94 & 98/90 \\
Stitched goals, PointMaze-M, budget 600 & 99 & 100/98 \\
Stitched goals, PointMaze-M, budget 800 & 99 & 100/98 \\
Reacher, mean over $d{=}25..150$ & 62 & 60/60/64/64 \\
\midrule
Data fraction 1\%, $d{=}200$ / stitched & 63 / 86 & 74/52 \\
Data fraction 2\%, $d{=}200$ / stitched & 80 / 73 & 86/74 \\
Data fraction 5\%, $d{=}200$ / stitched & 78 / 86 & 82/74 \\
Data fraction 10\%, $d{=}200$ / stitched & 79 / -- & 80/78 \\
Data fraction 25\%, $d{=}200$ / stitched & 83 / -- & 76/90 \\
Data fraction 50\%, $d{=}200$ / stitched & 84 / -- & 86/82 \\
Data fraction 100\%, $d{=}200$ / stitched & 86 / 94 & 92/80 \\


==> tables/supp_labels.tex <==
% generated by figs/scripts/export_labels.py from supp.aux; do not edit
\newlabel{app:phenomenon}{{A}{2}{}{}{}}
\newlabel{app:phenomenon@cref}{{[section][1][]A}{[1][2][]2}{}{}{}}
\newlabel{app:falls}{{A}{2}{}{}{}}
\newlabel{app:falls@cref}{{[section][1][]A}{[1][2][]2}{}{}{}}
\newlabel{app:published}{{A}{2}{}{}{}}
\newlabel{app:published@cref}{{[section][1][]A}{[1][2][]2}{}{}{}}
\newlabel{app:search}{{A}{2}{}{}{}}
\newlabel{app:search@cref}{{[section][1][]A}{[1][2][]2}{}{}{}}
\newlabel{app:closedloop}{{A}{2}{}{}{}}
\newlabel{app:closedloop@cref}{{[section][1][]A}{[1][2][]2}{}{}{}}
\newlabel{tab:published}{{S1}{2}{}{}{}}
\newlabel{tab:published@cref}{{[table][1][]S1}{[1][2][]2}{}{}{}}
\newlabel{app:graphs}{{B}{2}{}{}{}}
\newlabel{app:graphs@cref}{{[section][2][]B}{[1][2][]2}{}{}{}}
\newlabel{app:ranktest}{{B.1}{2}{}{}{}}
\newlabel{app:ranktest@cref}{{[subsection][1][2]B.1}{[1][2][]2}{}{}{}}
\newlabel{app:range}{{B.1}{2}{}{}{}}
\newlabel{app:range@cref}{{[subsection][1][2]B.1}{[1][2][]2}{}{}{}}
\newlabel{fig:e1range}{{S1}{3}{}{}{}}
\newlabel{fig:e1range@cref}{{[figure][1][]S1}{[1][3][]3}{}{}{}}
\newlabel{app:epochs}{{B.2}{3}{}{}{}}
\newlabel{app:epochs@cref}{{[subsection][2][2]B.2}{[1][3][]3}{}{}{}}
\newlabel{app:checks}{{B.3}{3}{}{}{}}
\newlabel{app:checks@cref}{{[subsection][3][2]B.3}{[1][3][]3}{}{}{}}
\newlabel{tab:truediag}{{S2}{3}{}{}{}}
\newlabel{tab:truediag@cref}{{[table][2][]S2}{[1][3][]3}{}{}{}}
\newlabel{fig:e1maps}{{S2}{4}{}{}{}}
\newlabel{fig:e1maps@cref}{{[figure][2][]S2}{[1][3][]4}{}{}{}}
\newlabel{fig:e2epochs}{{S3}{4}{}{}{}}
\newlabel{fig:e2epochs@cref}{{[figure][3][]S3}{[1][3][]4}{}{}{}}
\newlabel{app:theory}{{B.4}{5}{}{}{}}
\newlabel{app:theory@cref}{{[subsection][4][2]B.4}{[1][5][]5}{}{}{}}
\newlabel{lem:transfer}{{1}{5}{}{}{}}
\newlabel{lem:transfer@cref}{{[lemma][1][]1}{[1][5][]5}{}{}{}}
\newlabel{cor:true}{{1}{5}{}{}{}}
\newlabel{cor:true@cref}{{[corollary][1][]1}{[1][5][]5}{}{}{}}
\newlabel{prop:drift}{{1}{5}{}{}{}}
\newlabel{prop:drift@cref}{{[proposition][1][]1}{[1][5][]5}{}{}{}}
\newlabel{fig:diag}{{S4}{6}{}{}{}}
\newlabel{fig:diag@cref}{{[figure][4][]S4}{[1][5][]6}{}{}{}}
\newlabel{fig:hops}{{S5}{6}{}{}{}}
\newlabel{fig:hops@cref}{{[figure][5][]S5}{[1][5][]6}{}{}{}}
\newlabel{tab:driftt8}{{S3}{6}{}{}{}}
\newlabel{tab:driftt8@cref}{{[table][3][]S3}{[1][6][]6}{}{}{}}
\newlabel{app:predicts}{{B.5}{6}{}{}{}}
\newlabel{app:predicts@cref}{{[subsection][5][2]B.5}{[1][6][]6}{}{}{}}
\newlabel{app:focusmain}{{C}{7}{}{}{}}
\newlabel{app:focusmain@cref}{{[section][3][]C}{[1][7][]7}{}{}{}}
\newlabel{app:focus}{{C.1}{7}{}{}{}}
\newlabel{app:focus@cref}{{[subsection][1][3]C.1}{[1][7][]7}{}{}{}}
\newlabel{app:pushbias}{{C.2}{7}{}{}{}}
\newlabel{app:pushbias@cref}{{[subsection][2][3]C.2}{[1][7][]7}{}{}{}}
\newlabel{app:remedy}{{D}{7}{}{}{}}
\newlabel{app:remedy@cref}{{[section][4][]D}{[1][7][]7}{}{}{}}
\newlabel{app:remedyproof}{{D.1}{7}{}{}{}}
\newlabel{app:remedyproof@cref}{{[subsection][1][4]D.1}{[1][7][]7}{}{}{}}
\newlabel{fig:theory}{{S6}{8}{}{}{}}
\newlabel{fig:theory@cref}{{[figure][6][]S6}{[1][7][]8}{}{}{}}
\newlabel{app:method}{{D.2}{8}{}{}{}}
\newlabel{app:method@cref}{{[subsection][2][4]D.2}{[1][8][]8}{}{}{}}
\newlabel{alg:sga}{{S1}{8}{}{}{}}
\newlabel{alg:sga@cref}{{[algorithm][1][]S1}{[1][8][]8}{}{}{}}
\newlabel{alg:graph}{{S1}{8}{}{}{}}
\newlabel{alg:graph@cref}{{[algorithm][1][]S1}{[1][8][]8}{}{}{}}
\newlabel{alg:anchor}{{S1}{8}{}{}{}}
\newlabel{alg:anchor@cref}{{[algorithm][1][]S1}{[1][8][]8}{}{}{}}
\newlabel{alg:plan}{{S1}{8}{}{}{}}
\newlabel{alg:plan@cref}{{[algorithm][1][]S1}{[1][8][]8}{}{}{}}
\newlabel{fig:e1hops}{{S7}{9}{}{}{}}
\newlabel{fig:e1hops@cref}{{[figure][7][]S7}{[1][7][]9}{}{}{}}
\newlabel{tab:mw}{{S4}{10}{}{}{}}
\newlabel{tab:mw@cref}{{[table][4][]S4}{[1][8][]10}{}{}{}}
\newlabel{fig:exchange}{{S8}{10}{}{}{}}
\newlabel{fig:exchange@cref}{{[figure][8][]S8}{[1][7][]10}{}{}{}}
\newlabel{app:impl}{{D.3}{10}{}{}{}}
\newlabel{app:impl@cref}{{[subsection][3][4]D.3}{[1][10][]10}{}{}{}}
\newlabel{fig:suppgraph}{{S9}{11}{}{}{}}
\newlabel{fig:suppgraph@cref}{{[figure][9][]S9}{[1][8][]11}{}{}{}}
\newlabel{fig:suppanchor}{{S10}{11}{}{}{}}
\newlabel{fig:suppanchor@cref}{{[figure][10][]S10}{[1][8][]11}{}{}{}}
\newlabel{fig:suppcost}{{S11}{12}{}{}{}}
\newlabel{fig:suppcost@cref}{{[figure][11][]S11}{[1][10][]12}{}{}{}}
\newlabel{tab:graphs}{{S5}{12}{}{}{}}
\newlabel{tab:graphs@cref}{{[table][5][]S5}{[1][12][]12}{}{}{}}
\newlabel{app:results}{{E}{12}{}{}{}}
\newlabel{app:results@cref}{{[section][5][]E}{[1][12][]12}{}{}{}}
\newlabel{app:seeds}{{E.1}{12}{}{}{}}
\newlabel{app:seeds@cref}{{[subsection][1][5]E.1}{[1][12][]12}{}{}{}}
\newlabel{app:retrain}{{E.1}{12}{}{}{}}
\newlabel{app:retrain@cref}{{[subsection][1][5]E.1}{[1][12][]12}{}{}{}}
\newlabel{app:stats}{{E.1}{12}{}{}{}}
\newlabel{app:stats@cref}{{[subsection][1][5]E.1}{[1][12][]12}{}{}{}}
\newlabel{app:handoff}{{E.2}{12}{}{}{}}
\newlabel{app:handoff@cref}{{[subsection][2][5]E.2}{[1][12][]12}{}{}{}}
\newlabel{tab:compare}{{S6}{13}{}{}{}}
\newlabel{tab:compare@cref}{{[table][6][]S6}{[1][12][]13}{}{}{}}
\newlabel{fig:suppoptions}{{S12}{14}{}{}{}}
\newlabel{fig:suppoptions@cref}{{[figure][12][]S12}{[1][12][]14}{}{}{}}
\newlabel{tab:retrain}{{S7}{14}{}{}{}}
\newlabel{tab:retrain@cref}{{[table][7][]S7}{[1][12][]14}{}{}{}}
\newlabel{app:contactcfg}{{E.2}{14}{}{}{}}
\newlabel{app:contactcfg@cref}{{[subsection][2][5]E.2}{[1][14][]14}{}{}{}}
\newlabel{fig:plannerviewpusht}{{S13}{14}{}{}{}}
\newlabel{fig:plannerviewpusht@cref}{{[figure][13][]S13}{[1][14][]14}{}{}{}}
\newlabel{tab:contactcfg}{{S8}{14}{}{}{}}
\newlabel{tab:contactcfg@cref}{{[table][8][]S8}{[1][14][]14}{}{}{}}
\newlabel{app:ablations}{{E.3}{14}{}{}{}}
\newlabel{app:ablations@cref}{{[subsection][3][5]E.3}{[1][14][]14}{}{}{}}
\newlabel{fig:ablate}{{S14}{15}{}{}{}}
\newlabel{fig:ablate@cref}{{[figure][14][]S14}{[1][14][]15}{}{}{}}
\newlabel{tab:factorial}{{S9}{15}{}{}{}}
\newlabel{tab:factorial@cref}{{[table][9][]S9}{[1][15][]15}{}{}{}}
\newlabel{tab:search}{{S9}{15}{}{}{}}
\newlabel{tab:search@cref}{{[table][9][]S9}{[1][15][]15}{}{}{}}
\newlabel{tab:spanh}{{S10}{15}{}{}{}}
\newlabel{tab:spanh@cref}{{[table][10][]S10}{[1][15][]15}{}{}{}}
\newlabel{tab:stress}{{S11}{15}{}{}{}}
\newlabel{tab:stress@cref}{{[table][11][]S11}{[1][15][]15}{}{}{}}
\newlabel{app:beyond}{{E.4}{15}{}{}{}}
\newlabel{app:beyond@cref}{{[subsection][4][5]E.4}{[1][15][]15}{}{}{}}
\newlabel{fig:robust}{{S15}{16}{}{}{}}
\newlabel{fig:robust@cref}{{[figure][15][]S15}{[1][15][]16}{}{}{}}
\newlabel{app:baselines}{{E.5}{16}{}{}{}}
\newlabel{app:baselines@cref}{{[subsection][5][5]E.5}{[1][16][]16}{}{}{}}
\newlabel{tab:dwmcost}{{S12}{16}{}{}{}}
\newlabel{tab:dwmcost@cref}{{[table][12][]S12}{[1][16][]16}{}{}{}}
\newlabel{app:contemp}{{E.6}{17}{}{}{}}
\newlabel{app:contemp@cref}{{[subsection][6][5]E.6}{[1][17][]17}{}{}{}}
\newlabel{fig:pushtdist}{{S16}{17}{}{}{}}
\newlabel{fig:pushtdist@cref}{{[figure][16][]S16}{[1][17][]17}{}{}{}}
\newlabel{tab:pldm}{{S13}{18}{}{}{}}
\newlabel{tab:pldm@cref}{{[table][13][]S13}{[1][17][]18}{}{}{}}
\newlabel{tab:budget}{{S13}{18}{}{}{}}
\newlabel{tab:budget@cref}{{[table][13][]S13}{[1][17][]18}{}{}{}}
\newlabel{tab:graphpol}{{S14}{18}{}{}{}}
\newlabel{tab:graphpol@cref}{{[table][14][]S14}{[1][17][]18}{}{}{}}
\newlabel{tab:waypoint2}{{S14}{18}{}{}{}}
\newlabel{tab:waypoint2@cref}{{[table][14][]S14}{[1][17][]18}{}{}{}}
\newlabel{tab:contemp}{{S15}{19}{}{}{}}
\newlabel{tab:contemp@cref}{{[table][15][]S15}{[1][17][]19}{}{}{}}
\newlabel{tab:fidelity}{{S15}{19}{}{}{}}
\newlabel{tab:fidelity@cref}{{[table][15][]S15}{[1][17][]19}{}{}{}}
\newlabel{tab:metrosweep}{{S16}{19}{}{}{}}
\newlabel{tab:metrosweep@cref}{{[table][16][]S16}{[1][18][]19}{}{}{}}
\newlabel{tab:apoffset}{{S16}{19}{}{}{}}
\newlabel{tab:apoffset@cref}{{[table][16][]S16}{[1][18][]19}{}{}{}}
\newlabel{tab:comp_mech}{{S17}{20}{}{}{}}
\newlabel{tab:comp_mech@cref}{{[table][17][]S17}{[1][18][]20}{}{}{}}
\newlabel{tab:exec}{{S18}{21}{}{}{}}
\newlabel{tab:exec@cref}{{[table][18][]S18}{[1][21][]21}{}{}{}}
\newlabel{app:repro}{{E.7}{21}{}{}{}}
\newlabel{app:repro@cref}{{[subsection][7][5]E.7}{[1][21][]21}{}{}{}}
\newlabel{app:limits}{{F}{21}{}{}{}}
\newlabel{app:limits@cref}{{[section][6][]F}{[1][21][]21}{}{}{}}
\newlabel{fig:compquant}{{S17}{22}{}{}{}}
\newlabel{fig:compquant@cref}{{[figure][17][]S17}{[1][21][]22}{}{}{}}
\newlabel{app:qual}{{F.2}{22}{}{}{}}
\newlabel{app:qual@cref}{{[subsection][2][6]F.2}{[1][22][]22}{}{}{}}
\newlabel{fig:companatomy}{{S18}{23}{}{}{}}
\newlabel{fig:companatomy@cref}{{[figure][18][]S18}{[1][21][]23}{}{}{}}
\newlabel{fig:qual}{{S19}{24}{}{}{}}
\newlabel{fig:qual@cref}{{[figure][19][]S19}{[1][21][]24}{}{}{}}
\newlabel{fig:plannerview}{{S20}{24}{}{}{}}
\newlabel{fig:plannerview@cref}{{[figure][20][]S20}{[1][22][]24}{}{}{}}
\newlabel{tab:seedsx}{{S19}{25}{}{}{}}
\newlabel{tab:seedsx@cref}{{[table][19][]S19}{[1][21][]25}{}{}{}}


==> tables/table1_rows.tex <==
LeWM~\cite{maes2026leworldmodel} & 5 & 31 & 13 & 39 & 8 & 5 & 60 \\
LeWM + min-over-plan & 9 & 62 & 12 & 41 & 26 & 17 & 77 \\
PLDM~\cite{sobal2026learning} & 0 & 50 & 3 & 28 & 1 & 2 & 15 \\
DINO-WM~\cite{zhou2024dino}$^\ddagger$ & -- & 70 & 15 & 35 & \textbf{100} & \textbf{100} & -- \\
\midrule
GCBC~\cite{park2025ogbench} & 5 & \textbf{100}$^\dagger$ & 51 & 51 & 18 & 17 & 0 \\
GCIVL~\cite{park2025ogbench} & 0 & 81 & 0$^\dagger$ & 16 & 1 & 3 & 0 \\
GCIQL~\cite{park2025ogbench} & 0 & 37 & 1 & 12 & 3 & 3 & 0 \\
HILP~\cite{park2024foundation} & 0 & 87 & 1 & 18 & 9 & 10 & 0 \\
\midrule
\rowcolor{oursrow}\textbf{Graph Anchors (ours)} & 30 & 93 & 85 & \textbf{95} & 87 & 66 & 68 \\
\quad + switch cost & \textbf{48}$^\S$ & 83 & 77 & 84 & 92 & 66 & 73 \\
\quad + goal handoff & 35 & 87 & \textbf{86} & 86 & 86 & 61 & \textbf{80} \\


==> tables/timing_rows.tex <==
LeWM planner ($H{=}5$) & 1.45 & 0.79--1.47 \\
LeWM + min-over-plan ($H{=}10$) & 2.62 & 2.56--2.62 \\
\rowcolor{pactrow}Graph anchors ($H{=}10$) & 1.83 & 1.82--1.86 \\


==> tables/truediag_rows.tex <==
Push-T & 0.96 & 0.83 & 0.60 & 0.52 & 0.69 & 0.48 & 0.2 \\
Two-Room & 0.62 & 0.56 & 0.56 & -- & 0.26 & 0.27 & 0.0 \\
PointMaze-M & 0.98 & 0.66 & 0.32 & 0.48 & 0.82 & 0.27 & 0.0 \\
Reacher & 0.74 & 0.59 & 0.52 & 0.51 & 0.43 & 0.33 & -- \\
OGBench-Cube & 0.84 & 0.68 & 0.61 & 0.77 & 0.54 & 0.44 & -- \\


==> tables/waypoint2_rows.tex <==
GCBC & 83 & 55 & 51 & -- \\
GCBC + graph waypoints, $K{=}6$ & 82 & 43 & 57 & 0.4 \\
GCBC + graph waypoints, $K{=}2$ & 71 & 25 & 40 & 37.0 \\
\rowcolor{pactrow}Graph anchors + LeWM planner (ours) & 89 & 85 & 95 & -- \\


==> tables/waypoint2_rows_clean.tex <==
GCBC & 83 & 55 & 51 \\
GCBC + graph waypoints, $K{=}6$ & 82 & 43 & 57 \\
GCBC + graph waypoints, $K{=}2$ & 71 & 25 & 40 \\
\rowcolor{pactrow}Graph anchors + LeWM planner (ours) & 89 & 85 & 95 \\


==> tables/waypoint_rows.tex <==
GCBC & 94 & 80 & 58 & 38 & 56/52 \\
GCBC + graph waypoints & 94 & 86 & 58 & 34 & 58/50 \\
Graph anchors + LeWM planner (ours) & 90 & 84 & 88 & 92 & 98/90 \\

